On the mathematical structure of quantum models of computation based on Hamiltonian minimisation

Determining properties of ground states of spin Hamiltonians remains a topic of central relevance connecting disciplines of mathematical, theoretical and applied physics. In the last few decades, ground state properties of physical systems have been increasingly considered as computational resources. This thesis develops parts of the mathematical apparatus to create (program) ground states relevant for quantum and classical computation. The core findings presented in this thesis (now over a decade old) including that (i) logic operations (gates) can be embedded into the low-energy sector of Ising spins whereas three (and higher) body Ising interaction terms can be mimicked through the minimisation of 2- and 1-body Ising terms yet require the introduction of slack spins; (ii) Perturbation theory gadgets enable the emulation of interactions not present in a given Hamiltonian, e.g.~$YY$ interactions can be realized from $ZZ$, $XX$, the thesis contains a result from 2007 showing that physically relevant two-body model Hamiltonian's have a QMA-hard ground state energy decision problem. Merged with other results, this established that these models provide a universal resource for ground state quantum computation. More recent findings include the proof that an idealised version of the contemporary variational approach to quantum algorithms enables a universal model of quantum computation. Other related results are also presented as they relate to ground state quantum computation and the minimisation of Hamiltonians by quantum circuits. The topics covered include: Ising model reductions, stochastic versus quantum processes on graphs, quantum gates and circuits as tensor networks, variational quantum algorithms and Hamiltonian gadgets.

==> BoolAlgPost.tex <==
\newpage

\section{Boolean Algebra Postulates}

\begin{multicols}{2}

Identity Elements\\
$ x  \lor 0 = 0 $\\
$ x \land 1 = x $

Commutativity\\
$ x  \lor y = y \lor x $\\
$ x \land y = y \land x $

Complements\\
$ x  \lor  \overline{x} = 1 $\\
$ x \land \overline{x} = 0 $

Absorption\\
$ x \lor (x \land y) = x$\\
$ x \land (x \lor y) = x$\\
$ x \lor (\overline{x} \land y) = x \lor y$\\
$ x \land (\overline{x} \lor y) = x \land y$\\
$ (x \land y) \lor (x \land \overline{y}) = x$\\
$ (x \lor y) \land (x \lor \overline{y}) = x$ 

Consensus\\
$(x \land y) \lor (\overline{x} \land z) \lor (y \land z) = (x \land y) \lor (\overline{x}\land z)$
$(x \lor y) \land (\overline{x} \lor z) \land (y \lor z) = (x \lor y) \land (\overline{x}\lor z)$

\columnbreak

Associativity\\
$(x \lor y) \lor z = x \lor (y \lor z)$\\
$(x \land y) \land z = x \land (y \land z)$

Distributivity\\
$x \lor (y \land z) = (x \lor y) \land (x \lor z) $\\
$x \land (y \lor z) = (x \land y) \lor (x \land z) $

Idempotency\\
$x \lor x = x$\\
$x \land x = x$

Null elements\\
$x \lor 1 = 1$\\
$x \land 0 = 0$

Involution\\
$ \overline{(\overline{x})} = \overline{\overline{x}} = x $

De Morgan \footnote{De Morgan  Principle of Duality\\ Any theorem or postulate in Boolean algebra remains true if: \\ 0 $ \leftrightarrow $ 1\\
$ \land \leftrightarrow \lor $
}\\
 \noindent
$ \lnot(x \lor y) = \overline{x} \land \overline{y} $\\
$ \lnot(x \land y) = \overline{x} \lor \overline{y} $
\end{multicols}



    


==> DiracNotation.tex <==
\newpage

\section{Dirac Notation boot camp}\label{sec:dirac}
Let $\psi$ and $\phi$  be vectors in a $n$-dimensional complex vector space $\mathcal{V}$. We adopt Dirac notation in which  
\begin{equation*}
\psi\to\ket{\psi}, \quad \phi\to\ket{\phi}
\end{equation*}
and an inner product of these states is $\braket{\psi}{\phi}$. We assume that inner product is linear in the second argument and antilinear in the first, i.e.
\begin{eqnarray*}
\braket{\psi}{\alpha\phi_1+\beta\phi_2}=\alpha\braket{\psi}{\phi_1}+\beta\braket{\psi}{\phi_2},
\\
\braket{\alpha\psi_1+\beta\psi_2}{\phi}=\bar{\alpha}\braket{\psi_1}{\phi}+\bar{\beta}\braket{\psi_2}{\phi},
\end{eqnarray*}
where $\alpha, \beta \in \mathbb{C}$.
Every vector $\ket{\psi}\in\mathcal{V}$ can be expanded in the orthonormal basis $\{\ket{i}\}$:
\begin{equation*}
\ket{\psi}=\sum_i\alpha_i\ket{i}, \quad \alpha_i=\braket{i}{\psi} \in \mathbb{C}.
\end{equation*}

Let $A$ be a linear operator $A:\mathcal{V}\to\mathcal{V}$. In Dirac notations linear means
\begin{equation*}
A\big(\alpha\ket{\psi}+\beta\ket{\phi}\big)=\alpha A \ket{\psi}+\beta A \ket{\phi}.
\end{equation*}
Instead of $A\ket{\psi}$ we sometimes use $\ket{A\psi}$ or $\ket{A(\psi)}$.

\begin{myremark} (Linearity of the braket). As is typical in many schools of quantum physics, we observe linearity of the bracket as $\ket{A(\phi)} = A\ket{\phi}$ and $\ket{a\cdot \phi + b\cdot \psi}= a\cdot \ket{\phi} + b\cdot \ket{\psi}$. 
\end{myremark}

Let us define projectors onto unit vectors $\ket{\psi}$ as
\begin{equation}\label{eqn:DiracProjector}
P_{\psi}\bydef\ketbra{\psi}{\psi}.
\end{equation}
It is a projector as $P_{\psi}^2=\ket{\psi}\braket{\psi}\bra{\psi}=\ketbra{\psi}{\psi}=P_{\psi}$. Moreover, every Schmidt rank-1 projector in $\mathcal{V}$ can be represented in form \eqref{eqn:DiracProjector}.

\begin{myproblem} (Rank-1 projectors $\star$). 
A non-trivial operator $P$ is a Schmidt rank-1 projector if and only if it can be written as $\ketbra{\psi}{\psi}$. \\

\noindent {\bf Solution}. Let us write $P$ in terms of its singular value decomposition $P= UDV^\dagger$.  Assume $P$ is a projector.  Then $P^2 = P$ implies that 
\begin{equation}\label{eqn:svdP}
UDV^\dagger UDV^\dagger = UDV^\dagger
\end{equation}
and so $V^\dagger U = \eye$ and hence $V = U$.  We  further have from \eqref{eqn:svdP}  that $D^2=D$ and so $\text{spec}\{D\}\in \{0,1\}$. For $D$ rank-1, only a single eigenvalue is non-zero.  The eigenvalues of $D$ are monotonically ordered lexicographically in the standard basis. Hence $D = \ketbra{\bf 0}{\bf 0}$ and so $U\ketbra{\bf 0}{\bf 0}U^\dagger = \ketbra{\psi}{\psi}$. Note that an example of projector that has full rank $k$ is the $k\times k$ identity. One with rank $k-1$ is found considering $\eye - \ketbra{a}{a}$. 
\end{myproblem}

For every vector in orthonormal basis $\{\ket{i}\}$ we define a projector $P_i=\ketbra{i}{i}$ then
\begin{equation*}
\sum_i P_i\ket{\psi}=\sum_i \ketbra{i}{i} \sum_j\alpha_j\ket{j}=\sum_i\alpha_i\ket{i}=\ket{\psi},
\end{equation*}
i.e.
\begin{equation*}
\eye=\sum_i P_i,
\end{equation*}
where $\eye$ is the identity operator on $\mathcal{V}$.

Let $\mathcal{W}$ be a $m$-dimensional complex vector space. The vector $\ket{\psi}\otimes\ket{\phi}\in \mathcal{V}\otimes\mathcal{W}$, where $\ket{\psi}\in \mathcal{V},\ \ket{\phi}\in \mathcal{W}$. In Dirac notation it is 
\begin{equation*}
\ket{\psi}\ket{\phi}=\ket{\psi,\phi}\bydef\ket{\psi}\otimes\ket{\phi}.
\end{equation*}
If $A$ is a linear operator $A:\mathcal{V}\to\mathcal{V}$ and $B$ is a linear operator $B:\mathcal{W}\to\mathcal{W}$ then 
\begin{equation}
A\otimes B:\mathcal{V}\otimes\mathcal{W}\to\mathcal{V}\otimes\mathcal{W},
\quad
A\ket{\psi}\otimes B \ket{\phi}=\ket{A\psi}\ket{B\phi}.
\end{equation}


\begin{figure}[H]
  \centering
  \includegraphics[width=0.7\textwidth]{dirac_notation.JPG}
  \caption{Lifehack: how to save space using Dirac notation.} 
\label{fig:dirac_notation}
\end{figure}
\vspace{10pt}
\noindent




\subsection{Example: $\mathbb{C}^2$}
As an example let us consider vector space $\mathbb{C}^2$ with orthogonal basis vectors $\ket{0},\ket{1}$. A general state in $\mathbb{C}^2$ can then be written as 
\begin{equation}
\ket{\psi}= \cos(\theta) \ket{0} + e^{-i \phi}\sin(\theta) \ket{1}
\end{equation}
and we recall the 
Pauli operators defined by the following formulas
\begin{eqnarray*}
\eye = \ketbra{0}{0}+\ketbra{1}{1} = \sum \ketbra{a}{a},\qquad X = \ketbra{0}{1}+\ketbra{1}{0} = \sum \ketbra{1-a}{a},
\\
Y=-i\ketbra{0}{1}+i\ketbra{1}{0}=i\sum (-1)^a \ketbra{a}{1-a},\qquad Z = \ketbra{0}{0}-\ketbra{1}{1} = \sum (-1)^a\ketbra{a}{a}
\end{eqnarray*}
for $a\in \{0,1\}$. 

Hence if $\alpha\ket{0}+\beta\ket{1}$ is an eigenvector of $X$ and $\lambda$ is the corresponding eigenvalue then
\begin{equation*}
X(\alpha\ket{0}+\beta\ket{1})=\alpha\ket{1}+\beta\ket{0}=\lambda(\alpha\ket{0}+\beta\ket{1}).
\end{equation*}
And we come to the system of equations $\lambda\alpha=\beta$ and $\lambda\beta=\alpha$, which has two solutions $\lambda=\pm 1$. Consequently eigenvectors of $X$ are
\begin{equation*}
\ket{+}\bydef\frac{1}{\sqrt{2}}(\ket{0}+\ket{1}),\quad \ket{-}\bydef\frac{1}{\sqrt{2}}(\ket{0}-\ket{1}).
\end{equation*}

\begin{myproblem}
By using Dirac notation (i) find eigenvalues and eigenvectors of $Y,Z$. (ii) Show that 
\begin{equation*}
[X,Y]=2iZ,\quad [Y,Z]=2iX,\quad [Z,X]=2iY,
\end{equation*}
and hence (iii $\star$) show that $[\sigma_i, \sigma_j] = 2i\epsilon_{ijk}\sigma_k$, where $\epsilon$ is the Levi-Civita symbol, $\sigma_1=X,\sigma_2=Y$ and $\sigma_3=Z$. 
\end{myproblem}

Projectors on $\ket{0},\ket{1}$ states in Dirac notations are
\begin{equation*}
P_{0} \bydef  \ketbra{0}{0} = \frac{1}{2} (\mathds{1} + Z), \quad 
P_{1}\bydef \ketbra{1}{1} = \frac{1}{2} (\mathds{1} - Z).
\end{equation*}

 Projector on arbitrary state $\ket{\psi}=\alpha\ket{1}+\beta\ket{0}$
\begin{equation*}
P_{\psi} \bydef  \ketbra{\psi}{\psi} = \big(\alpha\ket{1}+\beta\ket{0}\big)\big(\alpha\bra{1}+\beta\bra{0}\big)=|\alpha|^2\ketbra{1}{1}+\alpha\bar{\beta}\ketbra{1}{0}+\bar{\alpha}\beta\ketbra{0}{1}+|\beta|^2\ketbra{0}{0}.
\end{equation*}
For example projector on $\ket{+}$ state in terms of ket-bra vectors of $\{0,1\}$ is equal to
\begin{equation*}
\ketbra{+}{+}=\frac{1}{2}\big(\ketbra{1}{1}+\ketbra{1}{0}+\ketbra{0}{1}+\ketbra{0}{0}\big).
\end{equation*}

\begin{myproblem}
Define iff statements on condition on the $a_{ij}$ terms for the operator 
\begin{equation}
\sum_{i, j\in \{0,1\}} a_{ij}\ketbra{i}{j}
\end{equation}
 to be (i) Hermitian and (ii) a projector. 
\end{myproblem}

Let us consider the tensor product of two eigenvectors of $X$ operator
\begin{equation*}
\ket{+-}=\frac{1}{\sqrt{2}}(\ket{0}+\ket{1})\otimes\frac{1}{\sqrt{2}}(\ket{0}-\ket{1})=\frac{1}{2}\big(\ket{00}-\ket{01}+\ket{10}-\ket{11}\big),
\end{equation*}
this state is in $\mathbb{C}\otimes\mathbb{C}$. In this space we can define so-called Bell states with entanglement property (see Problem \ref{pr:Entang})
\begin{equation*}
\ket{\Phi^{+}}=\frac{1}{\sqrt{2}}\big(\ket{00}+\ket{11}\big), \quad \ket{\Phi^{-}}=\frac{1}{\sqrt{2}}\big(\ket{00}-\ket{11}\big).
\end{equation*}

\begin{myproblem}
\begin{enumerate} 
\item[(1)] Show that the corresponding eigenvectors of the Pauli matrices $X, Y, Z$ are 
$\sqrt{2}\ket{\pm} = \ket{0}\pm \ket{1}$ and $\sqrt{2}\ket{y_\pm} = \ket{0}\pm i\cdot \ket{1}$ and $\ket{j}$ for $j=0,1$. 

\item[(2)]  Consider the operators $X\otimes X$, $Y\otimes Y$, $Z\otimes Z$. Use the tensor product to define an eigenbasis and calculate the eigenvalues for these same operators. 

\item[($\star$)] Find an eigenbasis for these same operators which can not be factorized using the tensor product.  (In quantum theory, these basis states are called, entangled.) 
\end{enumerate} 
\end{myproblem} 

\begin{myproblem}\label{pr:Entang}
Show that $\nexists \ket{\psi_1},\ket{\psi_2}\in \mathbb{C}^2$ for the Bell state to be expressed as $\ket{\Phi^{\pm}}=\ket{\psi_1\psi_2}$.  The states $\ket{\Phi^{\pm}}$ are therefore called entangled. 
\end{myproblem}

\begin{myproblem}(Bell basis). 
Using the right hand side equations, 
\begin{eqnarray*}
\sigma_0 = \sum \ketbra{a}{a},\qquad \sigma_1 = \sum \ketbra{1-a}{a},
\\
\sigma_2=i\sum (-1)^a \ketbra{a}{1-a},\qquad \sigma_3 =\sum (-1)^a\ketbra{a}{a}.
\end{eqnarray*}
for $a\in \{0,1\}$. 
Show that 
\begin{equation}
\frac{1}{\sqrt{2}}\left(\sum_{l\in\{0,1\}} \bra{l} \otimes \bra{l} \right) \sigma_i \otimes \eye = \frac{1}{\sqrt{2}}\sum_{l\in\{0,1\}} (\bra{l}\sigma_i) \otimes \bra{l}
\end{equation}
defines the Bell states (which defines an orthonormal basis in $\mathbb{C}^2\otimes \mathbb{C}^2$). Here $\sigma_i$ indexes the Pauli matrices. 
\end{myproblem}

\begin{myproblem}
Show that $P_1\otimes U + P_0\otimes \eye$ is unitary if and only if $U$ is unitary.  
\end{myproblem}

\begin{myproblem}
Show that $A^\dagger B^\dagger = B^\dagger A^\dagger$ if and only if $[A,B]=0$. 
\end{myproblem}






==> Dissertation/Makefile <==
all:
	latexmk -pdf -pdflatex="xelatex %O %S" dissertation
pdf:
	latexmk -pdf -jobname=synopsis_pdf -silent  dissertation.tex
draft:	
	pdflatex -ini -jobname="draft-preamble" "&pdflatex draft-preamble.tex\dump"
	latexmk -pdf -jobname=draft -silent --shell-escape draft.tex

clean:
	latexmk -C dissertation
	rm -f dissertation.bbl

distclean:
	## Core latex/pdflatex auxiliary files:
	rm -f *.aux
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.fls
	rm -f *.out
	rm -f *.toc

	## Intermediate documents:
	rm -f *.dvi
	rm -f *-converted-to.*
	# these rules might exclude image files for figures etc.
	# *.ps
	# *.eps
	# *.pdf

	## Bibliography auxiliary files (bibtex/biblatex/biber):
	rm -f *.bbl
	rm -f *.bcf
	rm -f *.blg
	rm -f *-blx.aux
	rm -f *-blx.bib
	rm -f *.brf
	rm -f *.run.xml

	## Build tool auxiliary files:
	rm -f *.fdb_latexmk
	rm -f *.synctex
	rm -f *.synctex.gz
	rm -f *.synctex.gz\(busy\)
	rm -f *.pdfsync

	## Auxiliary and intermediate files from other packages:

	# algorithms
	rm -f *.alg
	rm -f *.loa

	# achemso
	rm -f acs-*.bib

	# amsthm
	rm -f *.thm

	# beamer
	rm -f *.nav
	rm -f *.snm
	rm -f *.vrb

	#(e)ledmac/(e)ledpar
	rm -f *.end
	rm -f *.[1-9]
	rm -f *.[1-9][0-9]
	rm -f *.[1-9][0-9][0-9]
	rm -f *.[1-9]R
	rm -f *.[1-9][0-9]R
	rm -f *.[1-9][0-9][0-9]R
	rm -f *.eledsec[1-9]
	rm -f *.eledsec[1-9]R
	rm -f *.eledsec[1-9][0-9]
	rm -f *.eledsec[1-9][0-9]R
	rm -f *.eledsec[1-9][0-9][0-9]
	rm -f *.eledsec[1-9][0-9][0-9]R

	# glossaries
	rm -f *.acn
	rm -f *.acr
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls

	# gnuplottex
	rm -f *-gnuplottex-*

	# hyperref
	rm -f *.brf

	# knitr
	rm -f *-concordance.tex
	rm -f *.tikz
	rm -f *-tikzDictionary

	# listings
	rm -f *.lol

	# makeidx
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist

	# minitoc
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc[0-9]
	rm -f *.mtc[1-9][0-9]

	# minted
	rm -f _minted*
	rm -f *.pyg

	# morewrites
	rm -f *.mw

	# mylatexformat
	rm -f *.fmt

	# nomencl
	rm -f *.nlo

	# sagetex
	rm -f *.sagetex.sage
	rm -f *.sagetex.py
	rm -f *.sagetex.scmd

	# sympy
	rm -f *.sout
	rm -f *.sympy
	rm -f sympy-plots-for-*.tex/

	# pdfcomment
	rm -f *.upa
	rm -f *.upb

	#pythontex
	rm -f *.pytxcode
	rm -f pythontex-files-*/

	# Texpad
	rm -f .texpadtmp

	# TikZ & PGF
	rm -f *.dpth
	rm -f *.md5
	rm -f *.auxlock

	# todonotes
	rm -f *.tdo

	# xindy
	rm -f *.xdy

	# WinEdt
	rm -f *.bak
	rm -f *.sav

	# endfloat
	rm -f *.ttt
	rm -f *.fff
	rm -f *.aux
	rm -f *.bbl
	rm -f *.blg
	rm -f *.dvi
	rm -f *.fdb_latexmk
	rm -f *.fls
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.nav
	rm -f *.nlo
	rm -f *.out
	rm -f *.pdfsync
	rm -f *.ps
	rm -f *.snm
	rm -f *.synctex.gz
	rm -f *.toc
	rm -f *.vrb
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc0
	rm -f *.bak
	rm -f *.bcf
	rm -f *.run.xml


==> Dissertation/acronyms.tex <==
\chapter*{Acronyms}             % Заголовок
\addcontentsline{toc}{chapter}{Acronyms}  % Добавляем его в оглавление



\textbf{NISQ} - Noisy Intermediate Scale Quantum Technology 

\textbf{QAOA} - Quantum Approximate Optimization Algorithm 

\textbf{QAOA} - Quantum Alternating Operator Ansatz 

\textbf{QMA} - Quantum Merlin Author (analog of NP)

\textbf{VQE} - Variational Quantum Eigensolver (Algorithm) 


==> Dissertation/conclusion.tex <==
\chapter*{Заключение}						% Заголовок
\addcontentsline{toc}{chapter}{Заключение}	% Добавляем его в оглавление

%% Согласно ГОСТ Р 7.0.11-2011:
%% 5.3.3 В заключении диссертации излагают итоги выполненного исследования, рекомендации, перспективы дальнейшей разработки темы.
%% 9.2.3 В заключении автореферата диссертации излагают итоги данного исследования, рекомендации и перспективы дальнейшей разработки темы.
%% Поэтому имеет смысл сделать эту часть общей и загрузить из одного файла в автореферат и в диссертацию:

Основные результаты работы заключаются в следующем.
\input{common/concl}
И какая-нибудь заключающая фраза.


==> Dissertation/contents.tex <==
% Оглавление (ГОСТ Р 7.0.11-2011, 5.2)
\tableofcontents


==> Dissertation/dictionary.tex <==
\chapter*{Словарь терминов}             % Заголовок
\addcontentsline{toc}{chapter}{Словарь терминов}  % Добавляем его в оглавление

\textbf{TeX} - Cистема компьютерной вёрстки, разработанная американским профессором информатики Дональдом Кнутом

\textbf{Панграмма} - Короткий текст, использующий все или почти все буквы алфавита


==> Dissertation/dispackages-ps8lis21.tex <==
%%% Колонтитулы %%%
\usepackage{fancyhdr}

%%% Прикладные пакеты %%% 
\usepackage{calc}               % Пакет для расчётов параметров, например длины
%\usepackage{etoolbox}          % ради функции patchcmd для управления списком литературы

% Next line commented - PS 8lis21
%\usepackage {interfaces-base}   % Набор базовых интерфейсов к некоторым пакетам, конкретные реализации загружаются в стиле
\usepackage {interfaces-base-ps8lis21}   % Набор базовых интерфейсов к некоторым пакетам, конкретные реализации загружаются в стиле

%%% Заголовки %%%
\usepackage{titlesec}           % Пакет настройки шрифтов заголовков в тексте

%%% Оглавление %%%
\usepackage{tocloft}

%%% Счётчики %%%
\usepackage{chngcntr}           % оперативная перенастройка счётчиков

==> Dissertation/disstyles-ps8lis21.tex <==
%%% Изображения %%%
\graphicspath{{images/}{Dissertation/images/}}         % Пути к изображениям

% The next line commented - PS
%\LoadInterface {titlesec}                   % Подгружаем интерфейсы для дополнительных опций управления некоторыми пакетами

\usepackage{titlesec} % PS 8lis21

%%% Блок управления параметрами для выравнивания заголовков в тексте %%%
\newlength{\otstuplen}
\setlength{\otstuplen}{\theotstup\parindent}
\ifthenelse{\equal{\theheadingalign}{0}}{% выравнивание заголовков в тексте
    \newcommand{\hdngalign}{\filcenter}                % по центру
    \newcommand{\hdngaligni}{\hfill\hspace{\otstuplen}}% по центру
}{%
    \newcommand{\hdngalign}{\filright}                 % по левому краю
    \newcommand{\hdngaligni}{\hspace{\otstuplen}}      % по левому краю
} % В обоих случаях вроде бы без переноса, как и надо (ГОСТ Р 7.0.11-2011, 5.3.5)

%%% Оглавление %%%
\renewcommand{\cftchapdotsep}{\cftdotsep}                % отбивка точками до номера страницы начала главы/раздела
\renewcommand{\cfttoctitlefont}{\hdngaligni\fontsize{14pt}{16pt}\selectfont\bfseries}% вместе со следующей строкой
\renewcommand{\cftaftertoctitle}{\hfill}                 % устанавливает заголовок по центру
\setlength{\cftbeforetoctitleskip}{-1.4\curtextsize}     % Поскольку этот заголовок всегда является первым на странице, то перед ним отделять пустым тройным интервалом не следует. Независимо от основного шрифта, в этом случае зануление (почти) происходит при -1.4\curtextsize.
\setlength{\cftaftertoctitleskip}{\theintvl\curtextsize} % Если считаем Оглавление заголовком, то выставляем после него тройной интервал через наше определённое значение

%% Переносить слова в заголовке не допускается (ГОСТ Р 7.0.11-2011, 5.3.5). Заголовки в оглавлении должны точно повторять заголовки в тексте (ГОСТ Р 7.0.11-2011, 5.2.3). Прямого указания на запрет переносов в оглавлении нет, но по той же логике невнесения искажений в смысл, лучше в оглавлении не переносить:
\cftsetrmarg{2.55em plus1fil}                       %To have the (sectional) titles in the ToC, etc., typeset ragged right with no hyphenation
\renewcommand{\cftchappagefont}{\normalfont}        % нежирные номера страниц у глав в оглавлении
\renewcommand{\cftchapleader}{\cftdotfill{\cftchapdotsep}}% нежирные точки до номеров страниц у глав в оглавлении
%\renewcommand{\cftchapfont}{}                       % нежирные названия глав в оглавлении

\ifthenelse{\theheadingdelim > 0}{%
    \renewcommand\cftchapaftersnum{.\ }   % добавляет точку с пробелом после номера раздела в оглавлении
}{%
\renewcommand\cftchapaftersnum{\quad}     % добавляет \quad после номера раздела в оглавлении
}
\ifthenelse{\theheadingdelim > 1}{%
    \renewcommand\cftsecaftersnum{.\ }    % добавляет точку с пробелом после номера подраздела в оглавлении
    \renewcommand\cftsubsecaftersnum{.\ } % добавляет точку с пробелом после номера подподраздела в оглавлении
}{%
\renewcommand\cftsecaftersnum{\quad}      % добавляет \quad после номера подраздела в оглавлении
\renewcommand\cftsubsecaftersnum{\quad}   % добавляет \quad после номера подподраздела в оглавлении
}

\ifthenelse{\equal{\thepgnum}{1}}{%
%    \addtocontents{toc}{~\hfill{Стр.}\par}% добавить Стр. над номерами страниц %PS
\addtocontents{toc}{~\hfill{Page}\par}% добавить Стр. над номерами страниц
}

%%% Оформление названий глав %%%
%% настройки заголовка списка рисунков
\renewcommand{\cftloftitlefont}{\hdngaligni\fontsize{14pt}{16pt}\selectfont\bfseries}% вместе со следующей строкой
\renewcommand{\cftafterloftitle}{\hfill}                                             % устанавливает заголовок по центру
\setlength{\cftbeforeloftitleskip}{-1.5\curtextsize}     % Поскольку этот заголовок всегда является первым на странице, то перед ним отделять пустым тройным интервалом не следует. Независимо от основного шрифта, в этом случае зануление (почти) происходит при -1.5\curtextsize.
\setlength{\cftafterloftitleskip}{\theintvl\curtextsize} % выставляем после него тройной интервал через наше определённое значение

%% настройки заголовка списка таблиц
\renewcommand{\cftlottitlefont}{\hdngaligni\fontsize{14pt}{16pt}\selectfont\bfseries}% вместе со следующей строкой
\renewcommand{\cftafterlottitle}{\hfill}                                             % устанавливает заголовок по центру
\setlength{\cftbeforelottitleskip}{-1.5\curtextsize}     % Поскольку этот заголовок всегда является первым на странице, то перед ним отделять пустым тройным интервалом не следует. Независимо от основного шрифта, в этом случае зануление (почти) происходит при -1.5\curtextsize.
\setlength{\cftafterlottitleskip}{\theintvl\curtextsize} % выставляем после него тройной интервал через наше определённое значение

\ifnum\curtextsize>\bigtextsize     % Проверяем условие использования базового шрифта 14 pt
\setlength{\headheight}{17pt}       % Исправляем высоту заголовка
\else
\setlength{\headheight}{15pt}       % Исправляем высоту заголовка
\fi

%%% Колонтитулы %%%
% Порядковый номер страницы печатают на середине верхнего поля страницы (ГОСТ Р 7.0.11-2011, 5.3.8)
\makeatletter
\let\ps@plain\ps@fancy              % Подчиняем первые страницы каждой главы общим правилам
\makeatother
\pagestyle{fancy}                   % Меняем стиль оформления страниц
\fancyhf{}                          % Очищаем текущие значения
\fancyhead[C]{\thepage}             % Печатаем номер страницы на середине верхнего поля
\renewcommand{\headrulewidth}{0pt}  % Убираем разделительную линию

%%% Оформление заголовков глав, разделов, подразделов %%%
%% Работа должна быть выполнена ... размером шрифта 12-14 пунктов (ГОСТ Р 7.0.11-2011, 5.3.8). То есть не должно быть надписей шрифтом более 14. Так и поставим.
%% Эти установки будут давать одинаковый результат независимо от выбора базовым шрифтом 12 пт или 14 пт
%PS -- added \makeatletter
\makeatletter
\titleformat{\chapter}[block]                                % default display;  hang = with a hanging label. (Like the standard \section.); block = typesets the whole title in a block (a paragraph) without additional formatting. Useful in centered titles
        {\hdngalign\fontsize{14pt}{16pt}\selectfont\bfseries}% 
        %\fontsize{<size>}{<skip>} % второе число ставим 1.2*первое, чтобы адекватно отрабатывали команды по расчету полуторного интервала (домножая разные комбинации коэффициентов на этот)
        {\thechapter\cftchapaftersnum}                       % Заголовки в оглавлении должны точно повторять заголовки в тексте (ГОСТ Р 7.0.11-2011, 5.2.3).
        {0em}% отступ от номера до текста
        {}%

\titleformat{\section}[block]                                % default hang;  hang = with a hanging label. (Like the standard \section.); block = typesets the whole title in a block (a paragraph) without additional formatting. Useful in centered titles
        {\hdngalign\fontsize{14pt}{16pt}\selectfont\bfseries}% 
        %\fontsize{<size>}{<skip>} % второе число ставим 1.2*первое, чтобы адекватно отрабатывали команды по расчету полуторного интервала (домножая разные комбинации коэффициентов на этот)
        {\thesection\cftsecaftersnum}                        % Заголовки в оглавлении должны точно повторять заголовки в тексте (ГОСТ Р 7.0.11-2011, 5.2.3).
        {0em}% отступ от номера до текста
        {}%

\titleformat{\subsection}[block]                             % default hang;  hang = with a hanging label. (Like the standard \section.); block = typesets the whole title in a block (a paragraph) without additional formatting. Useful in centered titles
        {\hdngalign\fontsize{14pt}{16pt}\selectfont\bfseries}% 
        %\fontsize{<size>}{<skip>} % второе число ставим 1.2*первое, чтобы адекватно отрабатывали команды по расчету полуторного интервала (домножая разные комбинации коэффициентов на этот)
        {\thesubsection\cftsubsecaftersnum}                  % Заголовки в оглавлении должны точно повторять заголовки в тексте (ГОСТ Р 7.0.11-2011, 5.2.3).
        {0em}% отступ от номера до текста
        {}%

\ifthenelse{\equal{\thechapstyle}{1}}{%
    \sectionformat{\chapter}{% Параметры заголовков разделов в тексте
        label=\chaptername\ \thechapter\cftchapaftersnum,
        labelsep=0em,
    }
    %% Следующие две строки: будет вписано слово Глава перед каждым номером раздела в оглавлении   
    \renewcommand{\cftchappresnum}{\chaptername\ }
    \setlength{\cftchapnumwidth}{\widthof{\cftchapfont\cftchappresnum\thechapter\cftchapaftersnum}}
}%
\makeatother % PS 
%% Интервалы между заголовками
% На эти величины titlespacing множит через *
\beforetitleunit=\curtextsize% привязались к нашему размеру шрифта
\aftertitleunit=\curtextsize% привязались к нашему размеру шрифта

% Счётчик intvl и длина \otstup определены в файле setup
\titlespacing{\chapter}{\theotstup\parindent}{-1.7em}{*\theintvl}       % Заголовки отделяют от текста сверху и снизу тремя интервалами (ГОСТ Р 7.0.11-2011, 5.3.5). Поскольку название главы всегда является первым на странице, то перед ним отделять пустым тройным интервалом не следует. Независимо от основного шрифта, в этом случае зануление происходит при -1.7em.
\titlespacing{\section}{\theotstup\parindent}{*\theintvl}{*\theintvl}
\titlespacing{\subsection}{\theotstup\parindent}{*\theintvl}{*\theintvl}
\titlespacing{\subsubsection}{\theotstup\parindent}{*\theintvl}{*\theintvl}

%%% Блок дополнительного управления размерами заголовков
\ifthenelse{\equal{\theheadingsize}{1}}{% Пропорциональные заголовки и базовый шрифт 14 пт
    \renewcommand{\cfttoctitlefont}{\hdngaligni\Large\bfseries} % Исправляем размер заголовка оглавления
    \setlength{\cftbeforetoctitleskip}{-1.2\curtextsize}        % Исправляем вертикальный отступ перед заголовком оглавления
    \renewcommand{\cftloftitlefont}{\hdngaligni\Large\bfseries} % Исправляем размер заголовка списка рисунков
    \setlength{\cftbeforeloftitleskip}{-1.4\curtextsize}        % Исправляем вертикальный отступ перед заголовком списка рисунков
    \renewcommand{\cftlottitlefont}{\hdngaligni\Large\bfseries} % Исправляем размер заголовка списка таблиц 
    \setlength{\cftbeforelottitleskip}{-1.4\curtextsize}        % Исправляем вертикальный отступ перед заголовком списка таблиц
    \sectionformat{\chapter}{% Параметры заголовков разделов в тексте
        format=\hdngalign\Large\bfseries, % Исправляем размер заголовка
        top-=0.4em,                       % Исправляем вертикальный отступ перед заголовком
    }
    \sectionformat{\section}{% Параметры заголовков подразделов в тексте
        format=\hdngalign\large\bfseries, % Исправляем размер заголовка
    }
}

\ifthenelse{\equal{\theheadingsize}{1}\AND \curtextsize < \bigtextsize}{% Пропорциональные заголовки и базовый шрифт 14 пт
    \sectionformat{\chapter}{% Параметры заголовков разделов в тексте
        top-=0.2em, % Исправляем вертикальный отступ перед заголовком
    }
}

%%% Счётчики %%%

%% Упрощённые настройки шаблона диссертации: нумерация формул, таблиц, рисунков
\ifthenelse{\equal{\thecontnumeq}{1}}{%
    \counterwithout{equation}{chapter} % Убираем связанность номера формулы с номером главы/раздела
}
\ifthenelse{\equal{\thecontnumfig}{1}}{%
    \counterwithout{figure}{chapter}   % Убираем связанность номера рисунка с номером главы/раздела
}
\ifthenelse{\equal{\thecontnumtab}{1}}{%
    \counterwithout{table}{chapter}    % Убираем связанность номера таблицы с номером главы/раздела
}


%%http://www.linux.org.ru/forum/general/6993203#comment-6994589 (используется totcount)
\makeatletter
\def\formbytotal#1#2#3#4#5{%
    \newcount\@c
    \@c\totvalue{#1}\relax
    \newcount\@last
    \newcount\@pnul
    \@last\@c\relax
    \divide\@last 10
    \@pnul\@last\relax
    \divide\@pnul 10
    \multiply\@pnul-10
    \advance\@pnul\@last
    \multiply\@last-10
    \advance\@last\@c
    \total{#1}~#2%
    \ifnum\@pnul=1#5\else%
    \ifcase\@last#5\or#3\or#4\or#4\or#4\else#5\fi
    \fi
}
\makeatother

\AtBeginDocument{
%% регистрируем счётчики в системе totcounter
    \regtotcounter{totalcount@figure}
    \regtotcounter{totalcount@table}       % Если иным способом поставить в преамбуле то ошибка в числе таблиц
    \regtotcounter{TotPages}               % Если иным способом поставить в преамбуле то ошибка в числе страниц
}

==> Dissertation/draft.tex <==
%&draft-preamble
\begin{document}

% \input{../common/renames}             % Переопределение именований

% Структура диссертации (ГОСТ Р 7.0.11-2011, 4)
\include{title}           % Титульный лист
\include{contents}        % Оглавление
\subincludefrom{../}{introduction}    % Введение
\include{part1}           % Глава 1
\include{part2}           % Глава 2
\include{part3}           % Глава 3
\subincludefrom{../}{conclusion}      % Заключение
\include{acronyms}        % Список сокращений и условных обозначений
\include{dictionary}      % Словарь терминов
\include{references}      % Список литературы
\include{lists}           % Списки таблиц и изображений (иллюстративный материал)
\subincludefrom{../}{appendix}        % Приложения

\end{document}


==> Dissertation/introduction.tex <==
\chapter*{Introduction}							% Заголовок
\addcontentsline{toc}{chapter}{Introduction}	% Добавляем его в оглавление

\newcommand{\actuality}{}
\newcommand{\aim}{\textbf{Purpose of work}}
\newcommand{\tasks}{\textbf{tasks/problems}}
\newcommand{\defpositions}{\textbf{Key points for protection:}}
\newcommand{\novelty}{\textbf{Scientific novelty:}}
\newcommand{\influence}{\textbf{Scientific and practical relevance}}
\newcommand{\reliability}{\textbf{Confidence level}}
\newcommand{\probation}{\textbf{Work approbation.}}
\newcommand{\contribution}{\textbf{Personal contribution.}}
\newcommand{\publications}{\textbf{Publications.}}

\input{common/characteristic} % Характеристика работы по структуре во введении и в автореферате не отличается (ГОСТ Р 7.0.11, пункты 5.3.1 и 9.2.1), потому её загружаем из одного и того же внешнего файла, предварительно задав форму выделения некоторым параметрам

\textbf{Scope and structure of work.} The dissertation consists of introduction, four chapters, conclusion and two appendices. 
%% на случай ошибок оставляю исходный кусок на месте, закомментированным
%Полный объём диссертации составляет  \ref*{TotPages}~страницу с~\totalfigures{}~рисунками и~\totaltables{}~таблицами. Список литературы содержит \total{citenum}~наименований.
%
The full scope of the dissertation is \formbytotal{TotPages}{pages}{}{}{} 
including~\formbytotal{totalcount@figure}{figures}{}{}{}
and~\formbytotal{totalcount@table}{tables}{}{}{}.
Bibliography contains
\formbytotal{citenum}{items}{}{}{}.
% Полный объём диссертации составляет \formbytotal{TotPages}{страниц}{у}{ы}{} 
% с~\formbytotal{totalcount@figure}{рисунк}{ом}{ами}{ами}
% и~\formbytotal{totalcount@table}{таблиц}{ей}{ами}{ами}. Список литературы содержит  
% \formbytotal{citenum}{наименован}{ие}{ия}{ий}.


==> Dissertation/lists.tex <==
\clearpage
\phantomsection
\addcontentsline{toc}{chapter}{\listfigurename}
\listoffigures									% Список изображений


%%% Список таблиц %%%
% (ГОСТ Р 7.0.11-2011, 5.3.10)
\clearpage
\phantomsection
\addcontentsline{toc}{chapter}{\listtablename}
\listoftables									% Список таблиц
\newpage

==> Dissertation/part1.tex <==
\chapter{Оформление различных элементов} \label{chapt1}

\section{Форматирование текста} \label{sect1_1}

Мы можем сделать \textbf{жирный текст} и \textit{курсив}.

%\newpage
%============================================================================================================================

\section{Ссылки} \label{sect1_2}
Сошлёмся на библиографию. Одна ссылка: \cite[с.~54]{Sokolov}\cite[с.~36]{Gaidaenko}. Две ссылки: \cite{Sokolov,Gaidaenko}. Много ссылок:  \cite[с.~54]{Lermontov,Management,Borozda} \cite{Lermontov,Management,Borozda,Marketing,Constitution,FamilyCode,Gost.7.0.53,Razumovski,Lagkueva,Pokrovski,Sirotko,Lukina,Methodology,Encyclopedia,Nasirova,Berestova,Kriger}. И ещё немного ссылок: \cite{Article,Book,Booklet,Conference,Inbook,Incollection,Manual,Mastersthesis,Misc,Phdthesis,Proceedings,Techreport,Unpublished}. \cite{medvedev2006jelektronnye, CEAT:CEAT581, doi:10.1080/01932691.2010.513279,Gosele1999161,Li2007StressAnalysis, Shoji199895,test:eisner-sample,AB_patent_Pomerantz_1968,iofis_patent1960}

%Попытка реализовать несколько ссылок на конкретные страницы для стандартной реализации:[\citenum{Sokolov}, с.~54; \citenum{Gaidaenko}, с.~36].

%Несколько источников мультицитата \cites[vii--x, 5, 7]{Sokolov}[v--x, 25, 526]{Gaidaenko} поехали дальше

Ссылки на собственные работы:~\cite{vakbib1, confbib1}

Сошлёмся на приложения: Приложение \ref{AppendixA}, Приложение \ref{AppendixB2}.

Сошлёмся на формулу: формула \eqref{eq:equation1}.

Сошлёмся на изображение: рисунок \ref{img:knuth}.

%\newpage
%============================================================================================================================

\section{Формулы} \label{sect1_3}

Благодаря пакету \textit{icomma}, \LaTeX~одинаково хорошо воспринимает в качестве десятичного разделителя и запятую ($3,1415$), и точку ($3.1415$).

\subsection{Ненумерованные одиночные формулы} \label{subsect1_3_1}

Вот так может выглядеть формула, которую необходимо вставить в строку по тексту: $x \approx \sin x$ при $x \to 0$.

А вот так выглядит ненумерованая отдельностоящая формула c подстрочными и надстрочными индексами:
\[
(x_1+x_2)^2 = x_1^2 + 2 x_1 x_2 + x_2^2
\]

При использовании дробей формулы могут получаться очень высокие:
\[
  \frac{1}{\sqrt(2)+
  \displaystyle\frac{1}{\sqrt{2}+
  \displaystyle\frac{1}{\sqrt{2}+\cdots}}}
\]

В формулах можно использовать греческие буквы:
\[
\alpha\beta\gamma\delta\epsilon\varepsilon\zeta\eta\theta\vartheta\iota\kappa\lambda\\mu\nu\xi\pi\varpi\rho\varrho\sigma\varsigma\tau\upsilon\phi\varphi\chi\psi\omega\Gamma\Delta\Theta\Lambda\Xi\Pi\Sigma\Upsilon\Phi\Psi\Omega
\]

%\newpage
%============================================================================================================================

\subsection{Ненумерованные многострочные формулы} \label{subsect1_3_2}

Вот так можно написать две формулы, не нумеруя их, чтобы знаки равно были строго друг под другом:
\begin{align}
  f_W & =  \min \left( 1, \max \left( 0, \frac{W_{soil} / W_{max}}{W_{crit}} \right)  \right), \nonumber \\
  f_T & =  \min \left( 1, \max \left( 0, \frac{T_s / T_{melt}}{T_{crit}} \right)  \right), \nonumber
\end{align}

Выровнять систему ещё и по переменной $ x $ можно, используя окружение \verb|alignedat| из пакета \verb|amsmath|. Вот так: 
\[
    |x| = \left\{
    \begin{alignedat}{2}
        &&x, \quad &\text{eсли } x\geqslant 0 \\
        &-&x, \quad & \text{eсли } x<0
    \end{alignedat}
    \right.
\]
Здесь первый амперсанд  означает выравнивание по~левому краю, второй "--- по~$ x $, а~третий "--- по~слову <<если>>. Команда \verb|\quad| делает большой горизонтальный пробел. 

Ещё вариант:
\[
    |x|=
    \begin{cases}
    \phantom{-}x, \text{если } x \geqslant 0 \\
    -x, \text{если } x<0
    \end{cases}
\]

Можно использовать разные математические алфавиты:
\begin{align}
\mathcal{ABCDEFGHIJKLMNOPQRSTUVWXYZ} \nonumber \\
\mathfrak{ABCDEFGHIJKLMNOPQRSTUVWXYZ} \nonumber \\
\mathbb{ABCDEFGHIJKLMNOPQRSTUVWXYZ} \nonumber
\end{align}

Посмотрим на систему уравнений на примере аттрактора Лоренца:

\[ 
\left\{
  \begin{array}{rl}
    \dot x = & \sigma (y-x) \\
    \dot y = & x (r - z) - y \\
    \dot z = & xy - bz
  \end{array}
\right.
\]

А для вёрстки матриц удобно использовать многоточия:
\[ 
\left(
  \begin{array}{ccc}
  	a_{11} & \ldots & a_{1n} \\
  	\vdots & \ddots & \vdots \\
  	a_{n1} & \ldots & a_{nn} \\
  \end{array}
\right)
\]


%\newpage
%============================================================================================================================
\subsection{Нумерованные формулы} \label{subsect1_3_3}

А вот так пишется нумерованая формула:
\begin{equation}
  \label{eq:equation1}
  e = \lim_{n \to \infty} \left( 1+\frac{1}{n} \right) ^n
\end{equation}

Нумерованых формул может быть несколько:
\begin{equation}
  \label{eq:equation2}
  \lim_{n \to \infty} \sum_{k=1}^n \frac{1}{k^2} = \frac{\pi^2}{6}
\end{equation}

Впоследствии на формулы (\ref{eq:equation1}) и (\ref{eq:equation2}) можно ссылаться.

Сделать так, чтобы номер формулы стоял напротив средней строки, можно, используя окружение \verb|multlined| (пакет \verb|mathtools|) вместо \verb|multline| внутри окружения \verb|equation|. Вот так:
\begin{equation} % \tag{S} % tag - вписывает свой текст 
  \label{eq:equation3}
    \begin{multlined}
        1+ 2+3+4+5+6+7+\dots + \\ 
        + 50+51+52+53+54+55+56+57 + \dots + \\ 
        + 96+97+98+99+100=5050 
    \end{multlined}
\end{equation}

Используя команду \verb|\labelcref| из пакета \verb|cleveref|, можно
красиво ссылаться сразу на несколько формул
(\labelcref{eq:equation1,eq:equation3,eq:equation2}), даже перепутав
порядок ссылок \verb|(\labelcref{eq:equation1,eq:equation3,eq:equation2})|.


==> Dissertation/part2.tex <==
\chapter{Длинное название главы, в которой мы смотрим на примеры того, как будут верстаться изображения и списки} \label{chapt2}

\section{Одиночное изображение} \label{sect2_1}

\begin{figure}[ht] 
  \center
  \includegraphics [scale=0.27] {latex}
  \caption{TeX.} 
  \label{img:latex}  
\end{figure}

%\newpage
%============================================================================================================================
\section{Длинное название параграфа, в котором мы узнаём как сделать две картинки с общим номером и названием} \label{sect2_2}

А это две картинки под общим номером и названием:
\begin{figure}[ht]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=0.5\linewidth]{knuth1} \\ а)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=0.5\linewidth]{knuth2} \\ б)}
  \end{minipage}
  \caption{Очень длинная подпись к изображению, на котором представлены две фотографии Дональда Кнута}
  \label{img:knuth}  
\end{figure}

Те~же~две картинки под~общим номером и~названием, но с автоматизированной нумерацей подрисунков посредством пакета \verb|subcaption|:
\begin{figure}[ht]
    \center{
        \hfill
        \subcaptionbox[List-of-Figures entry]{Первый подрисунок\label{img:knuth_2_1}} {\includegraphics[width=0.25\linewidth]{knuth1}}%
        \hfill       
        \subcaptionbox{Второй подрисунок\label{img:knuth_2_2}} {\includegraphics[width=0.25\linewidth]{knuth2}}
        \hfill
    }
    
    \onehalfspacing{% внутри окружения figure набитый текст идёт через одинарный интервал, потому применяем эту команду пакета setspace. Возможно это временный "костыль", до появления соответствующей настройки в преамбуле
    Подрисуночный текст, описывающий обозначения, например. Согласно ГОСТ 2.105, пункт 4.3.1, располагается перед наименованием рисунка.
    }
    \caption{Очень длинная подпись к второму изображению, на котором представлены две фотографии Дональда Кнута} % Этот текст попадает в названия рисунков в списке рисунков
    \label{img:knuth_2}  
\end{figure}


На рисунке~\ref{img:knuth_2_1} показан Дональд Кнут без головного убора. На рисунке~\ref{img:knuth_2}\subref*{img:knuth_2_2}  показан Дональд Кнут в головном уборе.

%\newpage
%============================================================================================================================
\section{Пример вёрстки списков} \label{sect2_3}

\noindent Нумерованный список:
\begin{enumerate}
  \item Первый пункт.
  \item Второй пункт.
  \item Третий пункт.
\end{enumerate}

\noindent Маркированный список:
\begin{itemize}
  \item Первый пункт.
  \item Второй пункт.
  \item Третий пункт.
\end{itemize}

\noindent Вложенные списки:
\begin{itemize}
  \item Имеется маркированный список.
  \begin{enumerate}
    \item В нём лежит нумерованный список,
    \item в котором
    \begin{itemize}
      \item лежит ещё один маркированный список.
    \end{itemize}    
  \end{enumerate}
\end{itemize}


\section{Пробелы}

В~русском наборе принято:
\begin{itemize}
    \item единицы измерения, знак процента отделять пробелами от~числа: 10~кВт, 15~\% (согласно ГОСТ 8.417, раздел 8);
    \item $\tg 20^\circ$, но: 20~${}^\circ$C (согласно ГОСТ 8.417, раздел 8);
    \item знак номера, параграфа отделять от~числа: №~5, \S~8;
    \item стандартные сокращения: т.\:е., и~т.\:д., и~т.\:п.;
    \item неразрывные пробелы в~предложениях.
\end{itemize}

\section{Математика}

Русская традиция начертания греческих букв отличается от~западной. Это исправляется серией \verb|\renewcommand|.
\begin{itemize}
    \item[До:] $ \epsilon \ge \phi$, $\phi \leq \epsilon$, $\kappa \in \emptyset$.
    \renewcommand{\epsilon}{\ensuremath{\varepsilon}}
    \renewcommand{\phi}{\ensuremath{\varphi}}
    \renewcommand{\kappa}{\ensuremath{\varkappa}}
    \renewcommand{\le}{\ensuremath{\leqslant}}
    \renewcommand{\leq}{\ensuremath{\leqslant}}
    \renewcommand{\ge}{\ensuremath{\geqslant}}
    \renewcommand{\geq}{\ensuremath{\geqslant}}
    \renewcommand{\emptyset}{\varnothing}
    \item[После:] $\epsilon \ge \phi$, $\phi \leq \epsilon$, $\kappa \in \emptyset$.
\end{itemize}

Кроме того, принято набирать греческие буквы вертикальными, что решается подключением пакета \verb|upgreek| (см. закомментированный блок в \verb|userpackages.tex|) и~аналогичным переопределением в преамбуле (см. закомментированный блок в \verb|userstyles.tex|).


\section{Кавычки}
В английском языке приняты одинарные и двойные кавычки в~виде ‘...’ и~“...”. В России приняты французские («...») и~немецкие („...“) кавычки (они называются «ёлочки» и~«лапки», соответственно). <<Лапки>> обычно используются внутри ,,ёлочек``, например, <<... наш гордый ,,Варяг``...>>.

Французкие левые и правые кавычки набираются
как лигатуры \verb|<<| и \verb|>>|, а~немецкие левые и правые кавычки набираются как лигатуры \verb|,,| и \verb|‘‘| (\verb|``|).

Вместо лигатур или команд с~активным символом "\ можно использовать команды \verb|\glqq| и \verb|\grqq| для набора немецких кавычек и команды \verb|\flqq| и \verb|\frqq| для набора французских кавычек. Они определены в пакете \verb|babel|.

\section{Тире}
%  babel+pdflatex по умолчанию, в polyglossia надо включать опцией (и перекомпилировать с удалением временных файлов)
Команда \verb|"---| используется для печати тире в тексте. Оно несколько короче английского длинного тире. Кроме того, команда задаёт небольшую жёсткую отбивку от слова, стоящего перед тире. При этом, само тире не отрывается от слова. После тире следует такая же отбивка от текста, как и перед тире. При наборе текста между словом и командой, за которым она следует, должен стоять пробел.

В составных словах, таких, как <<Закон Менделеева"--~Клапейрона>>, для печати тире надо использовать команду \verb|"--~|. Она ставит более короткое, по~сравнению с~английским, тире и позволяет делать переносы во втором слове. При~наборе текста команда \verb|"--~| не отделяется пробелом от слова, за которым она следует (\verb|Менделеева"--~|). Следующее за командой слово может быть  отделено от~неё пробелом или перенесено на другую строку.

Если прямая речь начинается с~абзаца, то перед началом её печатается тире командой
\verb|"--*|. Она печатает русское тире и жёсткую отбивку нужной величины перед текстом.

\section{Дефисы и переносы слов}
%  babel+pdflatex по умолчанию, в polyglossia надо включать опцией (и перекомпилировать с удалением временных файлов)
Для печати дефиса в~составных словах введены две команды. Команда~\verb|"~| печатает дефис и~запрещает делать переносы в~самих словах, а~команда \verb|"=| печатает дефис, оставляя \TeX ’у право делать переносы в~самих словах.

В отличие от команды \verb|\-|, команда \verb|"-| задаёт место в~слове, где можно делать перенос, не~запрещая переносы и~в~других местах слова.

Команда \verb|""| задаёт место в~слове, где можно делать перенос, причём дефис при~переносе в~этом месте не~ставится.

Команда \verb|",| вставляет небольшой пробел после инициалов с~правом переноса в~фамилии.

\section{Текст из панграмм и формул}

Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг! Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен шляп (юфть) "--- вдрызг!Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф? Плюш изъят. Бьём чуждый цен хвощ! Эх, чужак! Общий съём цен

Ку кхоро адолэжкэнс волуптариа хаж, вим граэко ыкчпэтында ты. Граэкы жэмпэр льюкяльиюч квуй ку, аэквюы продыжщэт хаж нэ. Вим ку магна пырикульа, но квюандо пожйдонёюм про. Квуй ат рыквюы ёнэрмйщ. Выро аккузата вим нэ.
\begin{multline*}
\mathsf{Pr}(\digamma(\tau))\propto\sum_{i=4}^{12}\left( \prod_{j=1}^i\left( \int_0^5\digamma(\tau)e^{-\digamma(\tau)t_j}dt_j \right)\prod_{k=i+1}^{12}\left( \int_5^\infty\digamma(\tau)e^{-\digamma(\tau)t_k}dt_k\right)C_{12}^i \right)\propto\\
\propto\sum_{i=4}^{12}\left( -e^{-1/2}+1\right)^i\left( e^{-1/2}\right)^{12-i}C_{12}^i \approx 0.7605,\quad \forall\tau\neq\overline{\tau}
\end{multline*}
Квуй ыёюз омниюм йн. Экз алёквюам кончюлату квуй, ты альяквюам ёнвидюнт пэр. Зыд нэ коммодо пробатуж. Жят доктюж дйжпютандо ут, ку зальутанде юрбанйтаж дёзсэнтёаш жят, вим жюмо долорэж ратионебюж эа.

Ад ентэгры корпора жплэндидэ хаж. Эжт ат факэтэ дычэрунт пэржыкюти. Нэ нам доминг пэрчёус. Ку квюо ёужто эррэм зючкёпит. Про хабэо альбюкиюс нэ.
\[
\begin{pmatrix}
a_{11} & a_{12} & a_{13} \\
a_{21} & a_{22} & a_{23}
\end{pmatrix}
\]

\[
\begin{vmatrix}
a_{11} & a_{12} & a_{13} \\
a_{21} & a_{22} & a_{23}
\end{vmatrix}
\]

\[
\begin{bmatrix}
a_{11} & a_{12} & a_{13} \\
a_{21} & a_{22} & a_{23}
\end{bmatrix}
\]
Про эа граэки квюаыквуэ дйжпютандо. Ыт вэл тебиквюэ дэфянятйоныс, нам жолюм квюандо мандамюч эа. Эож пауло лаудым инкедыринт нэ, пэрпэтюа форынчйбюж пэр эю. Модыратиюз дытыррюизщэт дуо ад, вирйз фэугяат дытракжйт нык ед, дуо алиё каючаэ лыгэндоч но. Эа мольлиз юрбанйтаж зигнёфэрумквюы эжт.

Про мандамюч кончэтытюр ед. Трётанё прёнкипыз зигнёфэрумквюы вяш ан. Ат хёз эквюедым щуавятатэ. Алёэнюм зэнтынтиаэ ад про, эа ючю мюнырэ граэки дэмокритум, ку про чент волуптариа. Ыльит дыкоры аляквюид еюж ыт. Ку рыбюм мюндй ютенам дуо.
\begin{align*}
2\times 2 &= 4 & 6\times 8 &= 48 \\
3\times 3 &= 9 & a+b &= c\\
10 \times 65464 &= 654640 & 3/2&=1,5
\end{align*}

\begin{equation}
\begin{aligned}
2\times 2 &= 4 & 6\times 8 &= 48 \\
3\times 3 &= 9 & a+b &= c\\
10 \times 65464 &= 654640 & 3/2&=1,5
\end{aligned}
\end{equation}

Пэр йн тальэ пожтэа, мыа ед попюльо дэбетиз жкрибэнтур. Йн квуй аппэтырэ мэнандря, зыд аляквюид хабымуч корпора йн. Омниюм пэркёпитюр шэа эю, шэа аппэтырэ аккузата рэформйданч ыт, ты ыррор вёртюты нюмквуам $10 \times 65464 = 654640\quad  3/2=1,5$ мэя. Ипзум эуежмод $a+b = c$ мальюизчыт ад дуо. Ад фэюгаят пытынтёюм адвыржаряюм вяш. Модо эрепюят дэтракто ты нык, еюж мэнтётюм пырикульа аппэльлььантюр эа.

Мэль ты дэлььынётё такематыш. Зэнтынтиаэ конклььюжионэмквуэ ан мэя. Вёжи лебыр квюаыквуэ квуй нэ, дуо зймюл дэлььиката ку. Ыам ку алиё путынт.

%Большая фигурная скобка только справа
\[\left.                                                          %ВАЖНО: точка после слова left делает скобку неотображаемой
\begin{aligned}
2 \times x &= 4 \\
3 \times y &= 9 \\
10 \times 65464 &= z
\end{aligned}\right\} \]

Конвынёры витюпырата но нам, тебиквюэ мэнтётюм позтюлант ед про. Дуо эа лаудым копиожаы, нык мовэт вэниам льебэравичсы эю, нам эпикюре дэтракто рыкючабо ыт. Вэрйтюж аккюжамюз ты шэа, дэбетиз форынчйбюж жкряпшэрит ыт прё. Ан еюж тымпор рыфэррэнтур, ючю дольор котёдиэквюэ йн. Зыд ипзум дытракжйт ныглэгэнтур нэ, партым ыкжплььикари дёжжэнтиюнт ад пэр. Мэль ты кытэрож молыжтйаы, нам но ыррор жкрипта аппарэат.

\[ \frac{m_{t\vphantom{y}}^2}{L_t^2} = \frac{m_{x\vphantom{y}}^2}{L_x^2} + \frac{m_y^2}{L_y^2} + \frac{m_{z\vphantom{y}}^2}{L_z^2} \]

Вэре льаборэж тебиквюэ хаж ут. Ан пауло торквюатоз хаж, нэ пробо фэугяат такематыш шэа. Мэльёуз пэртинакёа юлламкорпэр прё ад, но мыа рыквюы конкыптам. Хёз квюот пэртинакёа эи, ельлюд трактатоз пэр ад. Зыд ед анёмал льаборэж номинави, жят ад конгуы льабятюр. Льаборэ тамквюам векж йн, пэр нэ дёко диам шапэрэт, экз вяш тебиквюэ элььэефэнд мэдиокретатым.

Нэ про натюм фюйзчыт квюальизквюэ, аэквюы жкаывола мэль ку. Ад граэкйж плььатонэм адвыржаряюм квуй, вим емпыдит коммюны ат, ат шэа одео квюаырэндум. Вёртюты ажжынтиор эффикеэнди эож нэ, доминг лаборамюз эи ыам. Чэнзэрет мныжаркхюм экз эож, ыльит тамквюам факильизиж нык эи. Квуй ан элыктрам тинкидюнт ентырпрытаряш. Йн янвыняры трактатоз зэнтынтиаэ зыд. Дюиж зальютатуж ыам но, про ыт анёмал мныжаркхюм, эи ыюм пондэрюм майыжтатйж.


==> Dissertation/part3.tex <==
\chapter{Вёрстка таблиц} \label{chapt3}

\section{Таблица обыкновенная} \label{sect3_1}

Так размещается таблица:

\begin{table} [htbp]
  \centering
  \parbox{15cm}{%
      \caption{Название таблицы}\label{Ts0Sib}%
  }
%  \begin{center}
  \begin{tabular}{| p{3cm} || p{3cm} | p{3cm} | p{4cm}l |}
  \hline
  \hline
  Месяц   & \centering $T_{min}$, К & \centering $T_{max}$, К &\centering  $(T_{max} - T_{min})$, К & \\
  \hline
  Декабрь &\centering  253.575   &\centering  257.778    &\centering      4.203  &   \\
  Январь  &\centering  262.431   &\centering  263.214    &\centering      0.783  &   \\
  Февраль &\centering  261.184   &\centering  260.381    &\centering     $-$0.803  &   \\
  \hline
  \hline
  \end{tabular}
%  \end{center}
\end{table}

\begin{table} [htbp]% Пример записи таблицы с номером, но без отображаемого наименования
	\centering
	\parbox{9cm}{% чтобы лучше смотрелось, подбирается самостоятельно
        \captionsetup{format=tablenocaption}% должен стоять до самого caption
        \caption{}%
        \label{tbl:test1}%
    	\begin{tabular}{ | c | c | c | c |}
    	\hline
    	Оконная функция	& ${2N}$ & ${4N}$	& ${8N}$	\\ \hline
    	Прямоугольное 	& 8.72 	 & 8.77		& 8.77		\\ \hline
    	Ханна		& 7.96 	 & 7.93		& 7.93		\\ \hline
    	Хэмминга	& 8.72 	 & 8.77		& 8.77		\\ \hline
    	Блэкмана	& 8.72 	 & 8.77		& 8.77		\\ \hline
    	\end{tabular}%
	}
\end{table}

Таблица \ref{tbl:test2} "--- пример таблицы, оформленной в~классическом книжном варианте или~очень близко к~нему. \mbox{ГОСТу} по~сути не~противоречит. Можно ещё~улучшить представление, с~помощью пакета \verb|siunitx| или~подобного.

\begin{table} [htbp]%
    \centering
	\caption{Наименование таблицы, очень длинное наименование таблицы, чтобы посмотреть как оно будет располагаться на~нескольких строках и~переноситься}%
	\label{tbl:test2}% label всегда желательно идти после caption
    \renewcommand{\arraystretch}{1.5}%% Увеличение расстояния между рядами, для улучшения восприятия.
	\begin{tabular}{@{}@{\extracolsep{20pt}}llll@{}} %Вертикальные полосы не используются принципиально, как и лишние горизонтальные (допускается по ГОСТ 2.105 пункт 4.4.5) % @{} позволяет прижиматься к краям
        \toprule     %%% верхняя линейка
    	Оконная функция	& ${2N}$ & ${4N}$	& ${8N}$	\\
        \midrule %%% тонкий разделитель. Отделяет названия столбцов. Обязателен по ГОСТ 2.105 пункт 4.4.5 
    	Прямоугольное 	& 8.72 	 & 8.77		& 8.77		\\
    	Ханна		& 7.96 	 & 7.93		& 7.93		\\
    	Хэмминга	& 8.72 	 & 8.77		& 8.77		\\
    	Блэкмана	& 8.72 	 & 8.77		& 8.77		\\
        \bottomrule %%% нижняя линейка
	\end{tabular}%
\end{table}

\section{Таблица с многострочными ячейками и примечанием}

Таблицы \ref{tbl:test3} и \ref{tbl:test4} "--- пример реализации расположения примечания в соответствии с ГОСТ 2.105. Каждый вариант со своими достоинствами и недостатками. Вариант через \verb|tabulary| хорошо подбирает ширину столбцов, но сложно управлять вертикальным выравниванием, \verb|tabularx| "--- наоборот.
\begin{table} [ht]%
	\caption{Нэ про натюм фюйзчыт квюальизквюэ}%
	\label{tbl:test3}% label всегда желательно идти после caption
    \setlength\extrarowheight{6pt} %вот этим управляем расстоянием между рядами, \arraystretch даёт неудачный результат
    \setlength{\tymin}{1.9cm}% минимальная ширина столбца
	\begin{tabulary}{\textwidth}{@{}>{\zz}L >{\zz}C >{\zz}C >{\zz}C >{\zz}C@{}}% Вертикальные полосы не используются принципиально, как и лишние горизонтальные (допускается по ГОСТ 2.105 пункт 4.4.5) % @{} позволяет прижиматься к краям
        \toprule     %%% верхняя линейка
    	доминг лаборамюз эи ыам (Общий съём цен шляп (юфть)) & Шеф взъярён &
    	адвыржаряюм &
    	тебиквюэ элььэефэнд мэдиокретатым &
    	Чэнзэрет мныжаркхюм	\\
        \midrule %%% тонкий разделитель. Отделяет названия столбцов. Обязателен по ГОСТ 2.105 пункт 4.4.5 
         Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф Плюш изъят. Бьём чуждый цен хвощ! &
        ${\approx}$ &
        ${\approx}$ &
        ${\approx}$ &
        $ + $ \\
        Эх, чужак! Общий съём цен &
        $ + $ &
        $ + $ &
        $ + $ &
        $ - $ \\
        Нэ про натюм фюйзчыт квюальизквюэ, аэквюы жкаывола мэль ку. Ад граэкйж плььатонэм адвыржаряюм квуй, вим емпыдит коммюны ат, ат шэа одео &
        ${\approx}$ &
        $ - $ &
        $ - $ &
        $ - $ \\
        Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. &
        $ - $ &
        $ + $ &
        $ + $ &
        ${\approx}$ \\
        Нэ про натюм фюйзчыт квюальизквюэ, аэквюы жкаывола мэль ку. Ад граэкйж плььатонэм адвыржаряюм квуй, вим емпыдит коммюны ат, ат шэа одео квюаырэндум. Вёртюты ажжынтиор эффикеэнди эож нэ. &
        $ + $ &
        $ - $ &
        ${\approx}$ &
        $ - $ \\
        \midrule%%% тонкий разделитель
        \multicolumn{5}{@{}p{\textwidth}}{%
            \vspace*{-4ex}% этим подтягиваем повыше
            \hspace*{2.5em}% абзацный отступ - требование ГОСТ 2.105
            Примечание "---  Плюш изъят: <<$+$>> "--- адвыржаряюм квуй, вим емпыдит; <<$-$>> "--- емпыдит коммюны ат; <<${\approx}$>> "--- Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф?
        }
        \\
        \bottomrule %%% нижняя линейка
	\end{tabulary}%
\end{table}

Из-за того, что таблица \ref{tbl:test3} не помещается на той же странице (при компилировании pdflatex), всё её содержимое переносится на следующую, ближайшую, а этот текст идёт перед ней.
\begin{table} [ht]%
	\caption{Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч}%
	\label{tbl:test4}% label всегда желательно идти после caption
    \renewcommand{\arraystretch}{1.6}%% Увеличение расстояния между рядами, для улучшения восприятия.
	\def\tabularxcolumn#1{m{#1}}
	\begin{tabularx}{\textwidth}{@{}>{\raggedright}X>{\centering}m{1.9cm} >{\centering}m{1.9cm} >{\centering}m{1.9cm} >{\centering\arraybackslash}m{1.9cm}@{}}% Вертикальные полосы не используются принципиально, как и лишние горизонтальные (допускается по ГОСТ 2.105 пункт 4.4.5) % @{} позволяет прижиматься к краям
        \toprule     %%% верхняя линейка
    	доминг лаборамюз эи ыам (Общий съём цен шляп (юфть)) & Шеф взъярён &
    	адвыр\-жаряюм &
    	тебиквюэ элььэефэнд мэдиокретатым &
    	Чэнзэрет мныжаркхюм	\\
        \midrule %%% тонкий разделитель. Отделяет названия столбцов. Обязателен по ГОСТ 2.105 пункт 4.4.5 
         Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф Плюш изъят. Бьём чуждый цен хвощ! &
        ${\approx}$ &
        ${\approx}$ &
        ${\approx}$ &
        $ + $ \\
        Эх, чужак! Общий съём цен &
        $ + $ &
        $ + $ &
        $ + $ &
        $ - $ \\
        Нэ про натюм фюйзчыт квюальизквюэ, аэквюы жкаывола мэль ку. Ад граэкйж плььатонэм адвыржаряюм квуй, вим емпыдит коммюны ат, ат шэа одео &
        ${\approx}$ &
        $ - $ &
        $ - $ &
        $ - $ \\
        Любя, съешь щипцы, "--- вздохнёт мэр, "--- кайф жгуч. &
        $ - $ &
        $ + $ &
        $ + $ &
        ${\approx}$ \\
        Нэ про натюм фюйзчыт квюальизквюэ, аэквюы жкаывола мэль ку. Ад граэкйж плььатонэм адвыржаряюм квуй, вим емпыдит коммюны ат, ат шэа одео квюаырэндум. Вёртюты ажжынтиор эффикеэнди эож нэ. &
        $ + $ &
        $ - $ &
        ${\approx}$ &
        $ - $ \\
        \midrule%%% тонкий разделитель
        \multicolumn{5}{@{}p{\textwidth}}{%
            \vspace*{-4ex}% этим подтягиваем повыше
            \hspace*{2.5em}% абзацный отступ - требование ГОСТ 2.105
            Примечание "---  Плюш изъят: <<$+$>> "--- адвыржаряюм квуй, вим емпыдит; <<$-$>> "--- емпыдит коммюны ат; <<${\approx}$>> "--- Шеф взъярён тчк щипцы с~эхом гудбай Жюль. Эй, жлоб! Где туз? Прячь юных съёмщиц в~шкаф. Экс-граф?
        }
        \\
        \bottomrule %%% нижняя линейка
	\end{tabularx}%
\end{table}

%\newpage
%============================================================================================================================

\section{Параграф - два} \label{sect3_2}

Некоторый текст.

%\newpage
%============================================================================================================================

\section{Параграф с подпараграфами} \label{sect3_3}

\subsection{Подпараграф - один} \label{subsect3_3_1}

Некоторый текст.

\subsection{Подпараграф - два} \label{subsect3_3_2}

Некоторый текст.

\clearpage

==> Dissertation/references.tex <==
\clearpage                                  % В том числе гарантирует, что список литературы в оглавлении будет с правильным номером страницы
\phantomsection
\addcontentsline{toc}{chapter}{\bibname}	% Добавляем список литературы в оглавление
%\hypersetup{ urlcolor=black }               % Ссылки делаем чёрными
%\providecommand*{\BibDash}{}                % В стилях ugost2008 отключаем использование тире как разделителя 
\urlstyle{rm}                               % ссылки URL обычным шрифтом
\insertbibliofull                          % Подключаем Bib-базы
\urlstyle{tt}                               % возвращаем установки шрифта ссылок URL
%\hypersetup{ urlcolor={urlcolor} }          % Восстанавливаем цвет ссылок

==> Dissertation/title.tex <==
% Титульный лист (ГОСТ Р 7.0.11-2001, 5.1)
\thispagestyle{empty}%
\begin{center}%
\MakeUppercase{\thesisOrganization}
\end{center}%
%
\vspace{0pt plus4fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{flushright}%
$\copyright$ 2020
\textsl {All Rights Reserved by the Author}
\end{flushright}%
%
\vspace{0pt plus6fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}%
{\large \thesisAuthor}
\end{center}%
%
\vspace{0pt plus1fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}%
\textbf {\large \thesisTitle}

\vspace{0pt plus2fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
{%\small
Speciality \\ 
``Theoretical Physics''~---~\thesisSpecialtyNumber\\
``\thesisSpecialtyTitle''
}

\vspace{0pt plus2fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
Dissertation for the degree of

\thesisDegree
\end{center}%
%
\vspace{0pt plus4fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{flushright}%
Supervisor:

\supervisorRegalia

\supervisorFio
\end{flushright}%
%
\vspace{0pt plus4fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}%
{\thesisCity~--- \thesisYear}
\end{center}%
\newpage


==> Dissertation/userstyles-ps.tex <==
% для вертикального центрирования ячеек в tabulary
\def\zz{\ifx\[$\else\aftergroup\zzz\fi}
\def\zzz{\setbox0\lastbox
\dimen0\dimexpr\extrarowheight + \ht0-\dp0\relax
\setbox0\hbox{\raise-.5\dimen0\box0}%
\ht0=\dimexpr\ht0+\extrarowheight\relax
\dp0=\dimexpr\dp0+\extrarowheight\relax 
\box0
}



\lstdefinelanguage{Renhanced}%
{keywords={abbreviate,abline,abs,acos,acosh,action,add1,add,%
        aggregate,alias,Alias,alist,all,anova,any,aov,aperm,append,apply,%
        approx,approxfun,apropos,Arg,args,array,arrows,as,asin,asinh,%
        atan,atan2,atanh,attach,attr,attributes,autoload,autoloader,ave,%
        axis,backsolve,barplot,basename,besselI,besselJ,besselK,besselY,%
        beta,binomial,body,box,boxplot,break,browser,bug,builtins,bxp,by,%
        c,C,call,Call,case,cat,category,cbind,ceiling,character,char,%
        charmatch,check,chol,chol2inv,choose,chull,class,close,cm,codes,%
        coef,coefficients,co,col,colnames,colors,colours,commandArgs,%
        comment,complete,complex,conflicts,Conj,contents,contour,%
        contrasts,contr,control,helmert,contrib,convolve,cooks,coords,%
        distance,coplot,cor,cos,cosh,count,fields,cov,covratio,wt,CRAN,%
        create,crossprod,cummax,cummin,cumprod,cumsum,curve,cut,cycle,D,%
        data,dataentry,date,dbeta,dbinom,dcauchy,dchisq,de,debug,%
        debugger,Defunct,default,delay,delete,deltat,demo,de,density,%
        deparse,dependencies,Deprecated,deriv,description,detach,%
        dev2bitmap,dev,cur,deviance,off,prev,,dexp,df,dfbetas,dffits,%
        dgamma,dgeom,dget,dhyper,diag,diff,digamma,dim,dimnames,dir,%
        dirname,dlnorm,dlogis,dnbinom,dnchisq,dnorm,do,dotplot,double,%
        download,dpois,dput,drop,drop1,dsignrank,dt,dummy,dump,dunif,%
        duplicated,dweibull,dwilcox,dyn,edit,eff,effects,eigen,else,%
        emacs,end,environment,env,erase,eval,equal,evalq,example,exists,%
        exit,exp,expand,expression,External,extract,extractAIC,factor,%
        fail,family,fft,file,filled,find,fitted,fivenum,fix,floor,for,%
        For,formals,format,formatC,formula,Fortran,forwardsolve,frame,%
        frequency,ftable,ftable2table,function,gamma,Gamma,gammaCody,%
        gaussian,gc,gcinfo,gctorture,get,getenv,geterrmessage,getOption,%
        getwd,gl,glm,globalenv,gnome,GNOME,graphics,gray,grep,grey,grid,%
        gsub,hasTsp,hat,heat,help,hist,home,hsv,httpclient,I,identify,if,%
        ifelse,Im,image,\%in\%,index,influence,measures,inherits,install,%
        installed,integer,interaction,interactive,Internal,intersect,%
        inverse,invisible,IQR,is,jitter,kappa,kronecker,labels,lapply,%
        layout,lbeta,lchoose,lcm,legend,length,levels,lgamma,library,%
        licence,license,lines,list,lm,load,local,locator,log,log10,log1p,%
        log2,logical,loglin,lower,lowess,ls,lsfit,lsf,ls,machine,Machine,%
        mad,mahalanobis,make,link,margin,match,Math,matlines,mat,matplot,%
        matpoints,matrix,max,mean,median,memory,menu,merge,methods,min,%
        missing,Mod,mode,model,response,mosaicplot,mtext,mvfft,na,nan,%
        names,omit,nargs,nchar,ncol,NCOL,new,next,NextMethod,nextn,%
        nlevels,nlm,noquote,NotYetImplemented,NotYetUsed,nrow,NROW,null,%
        numeric,\%o\%,objects,offset,old,on,Ops,optim,optimise,optimize,%
        options,or,order,ordered,outer,package,packages,page,pairlist,%
        pairs,palette,panel,par,parent,parse,paste,path,pbeta,pbinom,%
        pcauchy,pchisq,pentagamma,persp,pexp,pf,pgamma,pgeom,phyper,pico,%
        pictex,piechart,Platform,plnorm,plogis,plot,pmatch,pmax,pmin,%
        pnbinom,pnchisq,pnorm,points,poisson,poly,polygon,polyroot,pos,%
        postscript,power,ppoints,ppois,predict,preplot,pretty,Primitive,%
        print,prmatrix,proc,prod,profile,proj,prompt,prop,provide,%
        psignrank,ps,pt,ptukey,punif,pweibull,pwilcox,q,qbeta,qbinom,%
        qcauchy,qchisq,qexp,qf,qgamma,qgeom,qhyper,qlnorm,qlogis,qnbinom,%
        qnchisq,qnorm,qpois,qqline,qqnorm,qqplot,qr,Q,qty,qy,qsignrank,%
        qt,qtukey,quantile,quasi,quit,qunif,quote,qweibull,qwilcox,%
        rainbow,range,rank,rbeta,rbind,rbinom,rcauchy,rchisq,Re,read,csv,%
        csv2,fwf,readline,socket,real,Recall,rect,reformulate,regexpr,%
        relevel,remove,rep,repeat,replace,replications,report,require,%
        resid,residuals,restart,return,rev,rexp,rf,rgamma,rgb,rgeom,R,%
        rhyper,rle,rlnorm,rlogis,rm,rnbinom,RNGkind,rnorm,round,row,%
        rownames,rowsum,rpois,rsignrank,rstandard,rstudent,rt,rug,runif,%
        rweibull,rwilcox,sample,sapply,save,scale,scan,scan,screen,sd,se,%
        search,searchpaths,segments,seq,sequence,setdiff,setequal,set,%
        setwd,show,sign,signif,sin,single,sinh,sink,solve,sort,source,%
        spline,splinefun,split,sqrt,stars,start,stat,stem,step,stop,%
        storage,strstrheight,stripplot,strsplit,structure,strwidth,sub,%
        subset,substitute,substr,substring,sum,summary,sunflowerplot,svd,%
        sweep,switch,symbol,symbols,symnum,sys,status,system,t,table,%
        tabulate,tan,tanh,tapply,tempfile,terms,terrain,tetragamma,text,%
        time,title,topo,trace,traceback,transform,tri,trigamma,trunc,try,%
        ts,tsp,typeof,unclass,undebug,undoc,union,unique,uniroot,unix,%
        unlink,unlist,unname,untrace,update,upper,url,UseMethod,var,%
        variable,vector,Version,vi,warning,warnings,weighted,weights,%
        which,while,window,write,\%x\%,x11,X11,xedit,xemacs,xinch,xor,%
        xpdrows,xy,xyinch,yinch,zapsmall,zip},%
    otherkeywords={!,!=,~,$,*,\%,\&,\%/\%,\%*\%,\%\%,<-,<<-},%
    alsoother={._$},%
    sensitive,%
    morecomment=[l]\#,%
    morestring=[d]",%
    morestring=[d]'% 2001 Robert Denham
}%

%решаем проблему с кириллицей в комментариях (в pdflatex) https://tex.stackexchange.com/a/103712/79756
\lstset{extendedchars=true,literate={Ö}{{\"O}}1
    {Ä}{{\"A}}1
    {Ü}{{\"U}}1
    {ß}{{\ss}}1
    {ü}{{\"u}}1
    {ä}{{\"a}}1
    {ö}{{\"o}}1
    {~}{{\textasciitilde}}1
    {а}{{\selectfont\char224}}1
    {б}{{\selectfont\char225}}1
    {в}{{\selectfont\char226}}1
    {г}{{\selectfont\char227}}1
    {д}{{\selectfont\char228}}1
    {е}{{\selectfont\char229}}1
    {ё}{{\"e}}1
    {ж}{{\selectfont\char230}}1
    {з}{{\selectfont\char231}}1
    {и}{{\selectfont\char232}}1
    {й}{{\selectfont\char233}}1
    {к}{{\selectfont\char234}}1
    {л}{{\selectfont\char235}}1
    {м}{{\selectfont\char236}}1
    {н}{{\selectfont\char237}}1
    {о}{{\selectfont\char238}}1
    {п}{{\selectfont\char239}}1
    {р}{{\selectfont\char240}}1
    {с}{{\selectfont\char241}}1
    {т}{{\selectfont\char242}}1
    {у}{{\selectfont\char243}}1
    {ф}{{\selectfont\char244}}1
    {х}{{\selectfont\char245}}1
    {ц}{{\selectfont\char246}}1
    {ч}{{\selectfont\char247}}1
    {ш}{{\selectfont\char248}}1
    {щ}{{\selectfont\char249}}1
    {ъ}{{\selectfont\char250}}1
    {ы}{{\selectfont\char251}}1
    {ь}{{\selectfont\char252}}1
    {э}{{\selectfont\char253}}1
    {ю}{{\selectfont\char254}}1
    {я}{{\selectfont\char255}}1
    {А}{{\selectfont\char192}}1
    {Б}{{\selectfont\char193}}1
    {В}{{\selectfont\char194}}1
    {Г}{{\selectfont\char195}}1
    {Д}{{\selectfont\char196}}1
    {Е}{{\selectfont\char197}}1
    {Ё}{{\"E}}1
    {Ж}{{\selectfont\char198}}1
    {З}{{\selectfont\char199}}1
    {И}{{\selectfont\char200}}1
    {Й}{{\selectfont\char201}}1
    {К}{{\selectfont\char202}}1
    {Л}{{\selectfont\char203}}1
    {М}{{\selectfont\char204}}1
    {Н}{{\selectfont\char205}}1
    {О}{{\selectfont\char206}}1
    {П}{{\selectfont\char207}}1
    {Р}{{\selectfont\char208}}1
    {С}{{\selectfont\char209}}1
    {Т}{{\selectfont\char210}}1
    {У}{{\selectfont\char211}}1
    {Ф}{{\selectfont\char212}}1
    {Х}{{\selectfont\char213}}1
    {Ц}{{\selectfont\char214}}1
    {Ч}{{\selectfont\char215}}1
    {Ш}{{\selectfont\char216}}1
    {Щ}{{\selectfont\char217}}1
    {Ъ}{{\selectfont\char218}}1
    {Ы}{{\selectfont\char219}}1
    {Ь}{{\selectfont\char220}}1
    {Э}{{\selectfont\char221}}1
    {Ю}{{\selectfont\char222}}1
    {Я}{{\selectfont\char223}}1
    {і}{{\selectfont\char105}}1
    {ї}{{\selectfont\char168}}1
    {є}{{\selectfont\char185}}1
    {ґ}{{\selectfont\char160}}1
    {І}{{\selectfont\char73}}1
    {Ї}{{\selectfont\char136}}1
    {Є}{{\selectfont\char153}}1
    {Ґ}{{\selectfont\char128}}1
}

% Ширина текста минус ширина надписи 999
\newlength{\twless}
\newlength{\lmarg}
\setlength{\lmarg}{\widthof{999}}   % ширина надписи 999
\setlength{\twless}{\textwidth-\lmarg}


\lstset{ %
%    language=R,                     %  Язык указать здесь, если во всех листингах преимущественно один язык, в результате часть настроек может пойти только для этого языка
    numbers=left,                   % where to put the line-numbers
    numberstyle=\fontsize{12pt}{14pt}\selectfont\color{Gray},  % the style that is used for the line-numbers
    firstnumber=2,                  % в этой и следующей строках задаётся поведение нумерации 5, 10, 15...
    stepnumber=5,                   % the step between two line-numbers. If it's 1, each line will be numbered
    numbersep=5pt,                  % how far the line-numbers are from the code
    backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
    showspaces=false,               % show spaces adding particular underscores
    showstringspaces=false,         % underline spaces within strings
    showtabs=false,                 % show tabs within strings adding particular underscores
    frame=leftline,                 % adds a frame of different types around the code
    rulecolor=\color{black},        % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. commens (green here))
    tabsize=2,                      % sets default tabsize to 2 spaces
    captionpos=t,                   % sets the caption-position to top
    breaklines=true,                % sets automatic line breaking
    breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
%    title=\lstname,                 % show the filename of files included with \lstinputlisting;
    % also try caption instead of title
    basicstyle=\fontsize{12pt}{14pt}\selectfont\ttfamily,% the size of the fonts that are used for the code
%    keywordstyle=\color{blue},      % keyword style
    commentstyle=\color{ForestGreen}\emph,% comment style
    stringstyle=\color{Mahogany},   % string literal style
    escapeinside={\%*}{*)},         % if you want to add a comment within your code
    morekeywords={*,...},           % if you want to add more keywords to the set
    inputencoding=utf8,             % кодировка кода
    xleftmargin={\lmarg},           % Чтобы весь код и полоска с номерами строк была смещена влево, так чтобы цифры не вылезали за пределы текста слева
} 

%http://tex.stackexchange.com/questions/26872/smaller-frame-with-listings
% Окружение, чтобы листинг был компактнее обведен рамкой, если она задается, а не на всю ширину текста
\makeatletter
\newenvironment{SmallListing}[1][]
{\lstset{#1}\VerbatimEnvironment\begin{VerbatimOut}{VerbEnv.tmp}}
{\end{VerbatimOut}\settowidth\@tempdima{%
        \lstinputlisting{VerbEnv.tmp}}
    \minipage{\@tempdima}\lstinputlisting{VerbEnv.tmp}\endminipage}    
\makeatother


\DefineVerbatimEnvironment% с шрифтом 12 пт
{Verb}{Verbatim}
{fontsize=\fontsize{12pt}{14pt}\selectfont}

\RawFloats[figure,table]            % Отмена установок пакета floatrow для всех флотов (плавающих окружений) выбранных типов или подтипов. А то будто мы зря задавали настройки подписей рисунков и таблиц. 


% PS commented because of a strange conflict
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\DeclareNewFloatType{ListingEnv}{
%    placement=htb,
%    within=chapter,
%    fileext=lol,
%    name=Листинг,
%}
%
%\captionsetup[ListingEnv]{
%    format=tablecaption,
%    labelsep=space,                 % Точка после номера листинга задается значением period
 %   singlelinecheck=off,
 %   font=onehalfspacing,
%    position=top,
%}


%\floatsetup[ListingEnv]{
 %   style=plaintop,
%    captionskip=4pt,
%}

%\captionsetup[lstlisting]{
%    format=tablecaption,
%    labelsep=space,                 % Точка после номера листинга задается значением period
%    singlelinecheck=off,
%    font=onehalfspacing,
%    position=top,
%}

%\renewcommand{\lstlistingname}{Листинг}

%%Общие счётчики окружений листингов
%%http://tex.stackexchange.com/questions/145546/how-to-make-figure-and-listing-share-their-counter
%% Если смешивать плавающие и не плавающие окружения, то могут быть проблемы с нумерацией
%\makeatletter
%\AtBeginDocument{%
%    \let\c@ListingEnv\c@lstlisting
%    \let\theListingEnv\thelstlisting
%    \let\ftype@lstlisting\ftype@ListingEnv % give the floats the same precedence
%}
%\makeatother
%%%%%%%%%%%%%%%%%%%%%%%

% значок С++ — используйте команду \cpp
\newcommand{\cpp}{%
    C\nolinebreak\hspace{-.05em}%
    \raisebox{.2ex}{+}\nolinebreak\hspace{-.10em}%
    \raisebox{.2ex}{+}%
}


%%% Русская традиция начертания математических знаков
%\renewcommand{\le}{\ensuremath{\leqslant}}
%\renewcommand{\leq}{\ensuremath{\leqslant}}
%\renewcommand{\ge}{\ensuremath{\geqslant}}
%\renewcommand{\geq}{\ensuremath{\geqslant}}
%\renewcommand{\emptyset}{\varnothing}

%%% Русская традиция начертания греческих букв (греческие буквы вертикальные, через пакет upgreek)
%\renewcommand{\epsilon}{\ensuremath{\upvarepsilon}}   %  русская традиция записи
%\renewcommand{\phi}{\ensuremath{\upvarphi}}
%%\renewcommand{\kappa}{\ensuremath{\varkappa}}
%\renewcommand{\alpha}{\upalpha}
%\renewcommand{\beta}{\upbeta}
%\renewcommand{\gamma}{\upgamma}
%\renewcommand{\delta}{\updelta}
%\renewcommand{\varepsilon}{\upvarepsilon}
%\renewcommand{\zeta}{\upzeta}
%\renewcommand{\eta}{\upeta}
%\renewcommand{\theta}{\uptheta}
%\renewcommand{\vartheta}{\upvartheta}
%\renewcommand{\iota}{\upiota}
%\renewcommand{\kappa}{\upkappa}
%\renewcommand{\lambda}{\uplambda}
%\renewcommand{\mu}{\upmu}
%\renewcommand{\nu}{\upnu}
%\renewcommand{\xi}{\upxi}
%\renewcommand{\pi}{\uppi}
%\renewcommand{\varpi}{\upvarpi}
%\renewcommand{\rho}{\uprho}
%%\renewcommand{\varrho}{\upvarrho}
%\renewcommand{\sigma}{\upsigma}
%%\renewcommand{\varsigma}{\upvarsigma}
%\renewcommand{\tau}{\uptau}
%\renewcommand{\upsilon}{\upupsilon}
%\renewcommand{\varphi}{\upvarphi}
%\renewcommand{\chi}{\upchi}
%\renewcommand{\psi}{\uppsi}
%\renewcommand{\omega}{\upomega}


==> PSCyr/Synopsis/Makefile <==
all:
	latexmk -pdf -pdflatex="xelatex %O %S" synopsis

pdf:
	latexmk -pdf -jobname=synopsis_pdf -silent  synopsis.tex
# xedraft:
# 	xelatex -ini "&pdflatex draft-preamble.tex\dump"
# 	latexmk -pdf -pdflatex="xelatex %O %S" draft
draft:
	pdflatex -ini -jobname="draft-preamble" "&pdflatex draft-preamble.tex\dump"
	latexmk -pdf -jobname=draft -silent --shell-escape draft.tex

clean:
	latexmk -C synopsis
	rm -f synopsis.bbl

distclean:
	## Core latex/pdflatex auxiliary files:
	rm -f *.aux
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.fls
	rm -f *.out
	rm -f *.toc

	## Intermediate documents:
	rm -f *.dvi
	rm -f *-converted-to.*
	# these rules might exclude image files for figures etc.
	# *.ps
	# *.eps
	# *.pdf

	## Bibliography auxiliary files (bibtex/biblatex/biber):
	rm -f *.bbl
	rm -f *.bcf
	rm -f *.blg
	rm -f *-blx.aux
	rm -f *-blx.bib
	rm -f *.brf
	rm -f *.run.xml

	## Build tool auxiliary files:
	rm -f *.fdb_latexmk
	rm -f *.synctex
	rm -f *.synctex.gz
	rm -f *.synctex.gz\(busy\)
	rm -f *.pdfsync

	## Auxiliary and intermediate files from other packages:

	# algorithms
	rm -f *.alg
	rm -f *.loa

	# achemso
	rm -f acs-*.bib

	# amsthm
	rm -f *.thm

	# beamer
	rm -f *.nav
	rm -f *.snm
	rm -f *.vrb

	#(e)ledmac/(e)ledpar
	rm -f *.end
	rm -f *.[1-9]
	rm -f *.[1-9][0-9]
	rm -f *.[1-9][0-9][0-9]
	rm -f *.[1-9]R
	rm -f *.[1-9][0-9]R
	rm -f *.[1-9][0-9][0-9]R
	rm -f *.eledsec[1-9]
	rm -f *.eledsec[1-9]R
	rm -f *.eledsec[1-9][0-9]
	rm -f *.eledsec[1-9][0-9]R
	rm -f *.eledsec[1-9][0-9][0-9]
	rm -f *.eledsec[1-9][0-9][0-9]R

	# glossaries
	rm -f *.acn
	rm -f *.acr
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls

	# gnuplottex
	rm -f *-gnuplottex-*

	# hyperref
	rm -f *.brf

	# knitr
	rm -f *-concordance.tex
	rm -f *.tikz
	rm -f *-tikzDictionary

	# listings
	rm -f *.lol

	# makeidx
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist

	# minitoc
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc[0-9]
	rm -f *.mtc[1-9][0-9]

	# minted
	rm -f _minted*
	rm -f *.pyg

	# morewrites
	rm -f *.mw

	# mylatexformat
	rm -f *.fmt

	# nomencl
	rm -f *.nlo

	# sagetex
	rm -f *.sagetex.sage
	rm -f *.sagetex.py
	rm -f *.sagetex.scmd

	# sympy
	rm -f *.sout
	rm -f *.sympy
	rm -f sympy-plots-for-*.tex/

	# pdfcomment
	rm -f *.upa
	rm -f *.upb

	#pythontex
	rm -f *.pytxcode
	rm -f pythontex-files-*/

	# Texpad
	rm -f .texpadtmp

	# TikZ & PGF
	rm -f *.dpth
	rm -f *.md5
	rm -f *.auxlock

	# todonotes
	rm -f *.tdo

	# xindy
	rm -f *.xdy

	# WinEdt
	rm -f *.bak
	rm -f *.sav

	# endfloat
	rm -f *.ttt
	rm -f *.fff
	rm -f *.aux
	rm -f *.bbl
	rm -f *.blg
	rm -f *.dvi
	rm -f *.fdb_latexmk
	rm -f *.fls
	rm -f *.glg
	rm -f *.glo
	rm -f *.gls
	rm -f *.idx
	rm -f *.ilg
	rm -f *.ind
	rm -f *.ist
	rm -f *.lof
	rm -f *.log
	rm -f *.lot
	rm -f *.nav
	rm -f *.nlo
	rm -f *.out
	rm -f *.pdfsync
	rm -f *.ps
	rm -f *.snm
	rm -f *.synctex.gz
	rm -f *.toc
	rm -f *.vrb
	rm -f *.maf
	rm -f *.mtc
	rm -f *.mtc0
	rm -f *.bak
	rm -f *.bcf
	rm -f *.run.xml


==> PSCyr/Synopsis/content.tex <==
\subsection*{Общая характеристика работы}

\newcommand{\actuality}{\underline{\textbf{Актуальность темы.}}}
\newcommand{\aim}{\underline{\textbf{Целью}}}
\newcommand{\tasks}{\underline{\textbf{задачи}}}
\newcommand{\defpositions}{\underline{\textbf{Основные положения, выносимые на~защиту:}}}
\newcommand{\novelty}{\underline{\textbf{Научная новизна:}}}
\newcommand{\influence}{\underline{\textbf{Практическая значимость}}}
\newcommand{\reliability}{\underline{\textbf{Достоверность}}}
\newcommand{\probation}{\underline{\textbf{Апробация работы.}}}
\newcommand{\contribution}{\underline{\textbf{Личный вклад.}}}
\newcommand{\publications}{\underline{\textbf{Публикации.}}}

\input{common/characteristic} % Характеристика работы по структуре во введении и в автореферате не отличается (ГОСТ Р 7.0.11, пункты 5.3.1 и 9.2.1), потому её загружаем из одного и того же внешнего файла, предварительно задав форму выделения некоторым параметрам

%Диссертационная работа была выполнена при поддержке грантов ...

%\underline{\textbf{Объем и структура работы.}} Диссертация состоит из~введения, четырех глав, заключения и~приложения. Полный объем диссертации \textbf{ХХХ}~страниц текста с~\textbf{ХХ}~рисунками и~5~таблицами. Список литературы содержит \textbf{ХХX}~наименование.

%\newpage
\subsection*{Содержание работы}
Во \underline{\textbf{введении}} обосновывается актуальность исследований, проводимых в рамках данной диссертационной работы, приводится обзор научной литературы по изучаемой проблеме, формулируется цель, ставятся задачи работы, сформулированы научная новизна и практическая значимость представляемой работы.

\underline{\textbf{Первая глава}} посвящена ...

 картинку можно добавить так:
\begin{figure}[ht] 
  \center
  \includegraphics [scale=0.27] {latex}
  \caption{Подпись к картинке.} 
  \label{img:latex}
\end{figure}

Формулы в строку без номера добавляются так:
\[ 
  \lambda_{T_s} = K_x\frac{d{x}}{d{T_s}}, \qquad
  \lambda_{q_s} = K_x\frac{d{x}}{d{q_s}},
\]

\underline{\textbf{Вторая глава}} посвящена исследованию 

\underline{\textbf{Третья глава}} посвящена исследованию 

В \underline{\textbf{четвертой главе}} приведено описание 

В \underline{\textbf{заключении}} приведены основные результаты работы, которые заключаются в следующем:
\input{common/concl}


%\newpage
При использовании пакета \verb!biblatex! список публикаций автора по теме
диссертации формируется в разделе <<\publications>>\ файла
\verb!../common/characteristic.tex!  при помощи команды \verb!\nocite! 

\ifthenelse{\equal{\thebibliosel}{0}}{% Встроенная реализация с загрузкой файла через движок bibtex8
  \renewcommand{\refname}{\large \authorbibtitle}
  \nocite{*}
  \insertbiblioauthor                          % Подключаем Bib-базы
  %\insertbiblioother   % !!! bibtex не умеет работать с несколькими библиографиями !!!
}{% Реализация пакетом biblatex через движок biber
  \insertbiblioauthor                          % Подключаем Bib-базы
  \insertbiblioother
}



==> PSCyr/Synopsis/draft.tex <==
%&draft-preamble
\begin{document}

\input{title}           % Титульный лист
\subimport{../}{content}         % Содержание автореферата

\end{document}

==> PSCyr/Synopsis/setup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Файл упрощённых настроек шаблона диссертации %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%        Подключение пакетов                 %%%
\usepackage{ifthen}                 % добавляет ifthenelse
%%% Инициализирование переменных, не трогать!  %%%
\newcounter{bibliosel}
\newcounter{tabcap}
\newcounter{tablaba}
\newcounter{tabtita}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Область упрощённого управления оформлением %%%

%% Библиография

%% Внимание! При использовании bibtex8 необходимо удалить все
%% цитирования из  ../common/characteristic.tex 
\setcounter{bibliosel}{1}           % 0 --- встроенная реализация с загрузкой файла через движок bibtex8; 1 --- реализация пакетом biblatex через движок biber

%% Подпись таблиц
\setcounter{tabcap}{0}              % 0 --- по ГОСТ, номер таблицы и название разделены тире, выровнены по левому краю, при необходимости на нескольких строках; 1 --- подпись таблицы не по ГОСТ, на двух и более строках, дальнейшие настройки: 
%Выравнивание первой строки, с подписью и номером
\setcounter{tablaba}{2}             % 0 --- по левому краю; 1 --- по центру; 2 --- по правому краю
%Выравнивание строк с самим названием таблицы
\setcounter{tabtita}{1}             % 0 --- по левому краю; 1 --- по центру; 2 --- по правому краю

%%% Цвета гиперссылок %%%
% Latex color definitions: http://latexcolor.com/
\definecolor{linkcolor}{rgb}{0.9,0,0}
\definecolor{citecolor}{rgb}{0,0.6,0}
\definecolor{urlcolor}{rgb}{0,0,1}
%\definecolor{linkcolor}{rgb}{0,0,0} %black
%\definecolor{citecolor}{rgb}{0,0,0} %black
%\definecolor{urlcolor}{rgb}{0,0,0} %black

==> PSCyr/Synopsis/synpackages.tex <==
%%% Опционально %%%
% Следующий пакет может быть полезен, если надо ужать текст, чтобы сам текст не править, но чтобы места он занимал поменьше
%\usepackage{savetrees}

% Этот пакет может быть полезен для печати текста брошюрой
%\usepackage[print]{booklet}

==> PSCyr/Synopsis/synstyles.tex <==
%%% Изображения %%%
\graphicspath{{images/}{Synopsis/images/}}         % Пути к изображениям

%%% Макет страницы %%%
\oddsidemargin=-13pt
\topmargin=-66pt
\headheight=12pt
\headsep=38pt
\textheight=732pt
\textwidth=484pt
\marginparsep=14pt
\marginparwidth=43pt
\footskip=14pt
\marginparpush=7pt
\hoffset=0pt
\voffset=0pt
%\paperwidth=597pt
%\paperheight=845pt
\parindent=1.5cm                  % Размер табуляции (для красной строки) в начале каждого абзаца
\renewcommand{\baselinestretch}{1.25}

\newcommand{\sfs}{\fontsize{14pt}{15pt}\selectfont}
\sfs % размер шрифта и расстояния между строками


==> PSCyr/Synopsis/title.tex <==
\thispagestyle{empty}

\vspace{0pt plus1fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{flushright}
  \large{На правах рукописи}
  \includegraphics[height=1.5cm]{personal-signature} 
\end{flushright}

\vspace{0pt plus3fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}
\textbf {\large \thesisAuthor}
\end{center}

\vspace{0pt plus3fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}
\textbf {\Large \thesisTitle}

\vspace{0pt plus3fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
{\large Специальность \thesisSpecialtyNumber\ "---\par <<\thesisSpecialtyTitle>>}

\vspace{0pt plus1.5fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\Large{Автореферат}\par
\large{диссертации на соискание учёной степени\par \thesisDegree}
\end{center}

\vspace{0pt plus4fill} %число перед fill = кратность относительно некоторого расстояния fill, кусками которого заполнены пустые места
\begin{center}
{\large{\thesisCity\ "--- \thesisYear}}
\end{center}

\newpage
% оборотная сторона обложки
\thispagestyle{empty}
\noindent Работа выполнена в \thesisInOrganization

\par\bigskip
%\begin{table}[h] % считается не очень правильным использовать окружение table, не задавая caption
    \noindent%
    \begin{tabular}{@{}lp{11cm}}
        \sfs Научный руководитель: & \sfs \supervisorRegalia \par
                                      \textbf{\supervisorFio}
        \vspace{4mm} \\
        {\sfs Официальные оппоненты:} &
        {\sfs \textbf{\opponentOneFio,}\par
                  \opponentOneRegalia,\par
                  \opponentOneJobPlace,\par
                  \opponentOneJobPost\par \vspace{3mm}
                  \textbf{\opponentTwoFio,}\par \vspace{1mm}
                  \opponentTwoRegalia,\par
                  \opponentTwoJobPlace,\par
                  \opponentTwoJobPost
        }
        \vspace{4mm} \\
        {\sfs Ведущая организация:} & {\sfs \leadingOrganizationTitle }
    \end{tabular}  
%\end{table}
\par\bigskip

\noindent Защита состоится \defenseDate~на~заседании диссертационного совета \defenseCouncilNumber~на базе \defenseCouncilTitle~по адресу: \defenseCouncilAddress.

\vspace{5mm}
\noindent С диссертацией можно ознакомиться в библиотеке \synopsisLibrary.

\vspace{5mm}
\noindent{Автореферат разослан \synopsisDate.}

\vspace{5mm}
%\begin{table} [h] % считается не очень правильным использовать окружение table, не задавая caption
\par\bigskip
    \noindent%
    \begin{tabular}{p{8cm}cr}
        \begin{tabular}{p{8cm}}
            \sfs Ученый секретарь  \\
            \sfs диссертационного совета  \\
            \sfs \defenseCouncilNumber, \defenseSecretaryRegalia
        \end{tabular} 
    &
        \begin{tabular}{c}
            \includegraphics[height=1cm]{secretary-signature} 
        \end{tabular} 
    &
        \begin{tabular}{r}
            \\
            \\
            \sfs \defenseSecretaryFio
        \end{tabular} 
    \end{tabular}
%\end{table}
\newpage


==> PSCyr/pscyr/doc/PROBLEMS <==
This file explains how to solve some known problems occuring in PSCyr-0.4.

Q. dvips produces an error message "First number not found. ERROR in
   encoding vector in <...>".
A. Your dvips file is old.  Either upgrade to newer dvips (version 5.86
   or higher) or use your dvips with the -j0 option.

Q. Acrobat 4 issues the message "CRBUTR+AntiquaPSCyr-Bold contains a bad
   /BBox".
A. You have an old version of pdftex.  Upgrade to a newer one (current
   stable version is 0.14f).

Q. Acrobat 4 doesn't show the CourierPSMT-Italic font in PDF files
   produced by pdflatex.
A. Upgrade the fonts to PSCyr-0.4b or prepare your PDF file from PostScript
   using gs6** (tex->dvi->ps->pdf).

Q. Acrobat 4 issues the message "Unable to extract the embedded font
   'AACDDA+CourierPSMT-Italic'. Some characters may not display or print
   correctly" when reading PDF files produced by pdflatex.
A. Upgrade the fonts to PSCyr-0.4b or prepare your PDF file from PostScript
   using gs6** (tex->dvi->ps->pdf).

Q. TeX issues a warning like "Font shape `OMS/faq/m/n` undefined ..."
A. Ignore this message.  PSCyr font collection doesn't contain math and
   symbol characters that enter OMS, OML, OMX, and TS1 encoding tables.
   The required characters are taken from other fonts (like Computer Modern).

Q. TeX produces a wrong position of the ring in \AA symbol in all Russian
   fonts.
A. Comment the command "\DeclareTextCompositeCommand ..." in t2aenc.def file.


==> PSCyr/pscyr/doc/old/README.30 <==
NAME

    PSCYR package, version 0.3 from  September 10, 1998. 

DESCRIPTION 
   
    Collection of files providing support for Cyrillic 
    PostScript Fonts in LaTeX documents. 

    Final output is PostScript or PDF. 

DISTRIBUTION 

The distribution is split into two parts.

  * The first part (PsCyr-type1-03.tar.gz) 
    contains the files that are unlikely to change in 
    future releases:

    - font sources in Type 1 format;
    - Adobe font metrics.

    Fonts: Academy, Advertisement, Antiqua, College, Handbook,
       Lazurski, Magazine, Textbook, ArialCyrMT, CourierCyrPS,
       ERKurierKOI8RRegular, TimesNRCyrMT.

  * The second part (PsCyr-tex-03.tar.gz) 
    contains the files that are liable to modifications:
   
    - installation instructions (this file);
    - TeX font metrics;
    - font definitions; 
    - encodings; 
    - font mappings for DVIPS and pdfTeX
    - style and examples of usage;
    - scripts for generation of TeX font metrics and the map
      file.


INSTALLATION

  * Requirements

    - T2 package for LaTeX. This package is available from  
      CTAN:macros/latex/contrib/supported/t2. 
      It provides support for T2* Cyrillic TeX encodings. 
    - Dvips or pdf-LaTeX installed. Ghostscript (ghostview) or
      Acrobat Reader to visualize and print PostScript/PDF
      documents.


  * Procedure

     - Unpack the distribution: PsCyr-type1-[version].tar.gz,
                                PsCyr-tex-[version].tar.gz.

    TeX:
 
    - Copy the .tfm and .fd files to where TeX can find them.
    - Modify if necessary the TFMFONTS and TEXINPUTS environment
      variables.


    DVIPS:

    - Copy the .pfb and .enc files to where DVIPS headers reside.
    - Modify if necessary the DVIPSHEADERS environment variable. 
    - Add the string
         p +pscyr.map
      to the global configuration file config.ps, or
      to .dvipsrc in your home directory (UNIX).
    - Specify the path to pscyr.map in the TEXCONFIG environment
      variable.


    pdfTeX:
  
    - Copy the .pfb, .enc, and pscyr.map files to where pdfTeX
      headers reside.
    - Add the string
         map +pscyr.map
      to the global configuration file pdftex.cfg.
    - If you don't have permission to modify the global
      pdftex.cfg (UNIX), modify local copy and specify its 
      location in the TEXPSHEADERS environment variable.



USAGE 

  * LaTeX

Once the installation is made for LaTeX, Cyrillic PostScript
fonts become available in LaTeX documents. For example,
   
   \usefont{T2A}{faq}{m}{n} 

loads the Antiqua font at medium weight and upright shape.  You
may redefine the default font family by issuing the command

   \renewcommand{\rmdefault}{faq} 

in the header. See the examples provided and the style file
pscyr.sty. Also look at the font definitions for available
weights and shapes for different font families.


  * Printing and previewing

After the document is converted to PostScript by DVIPS, it can be
visualized and printed with ghostscript/ghostview.

++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
ATTENTION: Use DVIPS with -j0 option. Otherwise font re-encoding
           does not work properly.
++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

pdfLaTeX creates PDF directly from TeX source. This can be
printed and previewed with freely available Acrobat Reader.


  * Adding new fonts (UNIX only) 

You may use the perl scripts located in ./src to generate TeX
font metrics and the map file. These scripts are batch files for
afm2tfm program, which must be installed on your system. The
procedure is the following.

    - Copy Adobe font metrics of the new font to ./afm
   
    - Choose or create the appropriate encoding vector in ./enc.
    - Modify the file fontmap.txt in ./src. The syntax is

      TFM_NAME TMP_NAME AFM_NAME EFFECTS

      TFM_NAME : name of TeX font metrics file to create;
      TMP_NAME : unique name of temporary tfm file, which will be
                 created and erased by the script;
      AFM_NAME : name of Adobe font metrics file;

      EFFECTS  : E -extended, e - condensed, s - slanted. 
                 [012] - number of .enc file containing
                 the encoding vector.

    - Run the script make-all.sh. The .tfm and .map files will be
      created.

NOTES

The PSCYR package is unsupported, though serious bugs get fixed
somehow. The most serious problem is the quality of free fonts
included in the distribution: non-standard encodings, absent
ligatures, no kerning.

The typefaces included in this package originally come from   

    - The Monotype Corporation plc. (with changes by 
      Eugene V. Demidov);
    - Gavin Helf (with changes by Andrey A. Chernov);
    - ParaType, division of ParaGraph International.  

As to my knowledge, these fonts are placed into public domain and
can be freely redistributed.

COPYRIGHT 

The PSCYR package is free software provided "as is" without any
warranty.  You can redistribute it and/or modify it, provided
that the same notice appears in the modified version.


AUTHOR

Konstantin Chumachenko <chumachenko@writeme.com>;

thanks to:

Vladimir Volovich <TeX@vvv.vsu.ru>, for scripts and bug fixes;
Vitaly Repin <2:5030/209.26@fidonet.org>, for PSCYR style file. 
    


==> Warmup.tex <==
\section{Prerequisite Problems} \label{sec:Prerequisite}

In teaching this material to a variety of students in backgrounds 
ranging across the disciplines of Physics, Computer Science and Mathematics, 
it has proven helpful to begin the course with a few background problems related to some 
linear algebra and quantum physics concepts which relate to some of the ideas 
contained herein.  We typically assign such problems on the 
first day of a course and then have a worked problems session detailing 
all solutions shortly thereafter.  This increased student engagement, 
particularly for students coming from diverse backgrounds outside of physics.  

\begin{myproblem}[Hilbert spaces, projectors and spectral properties]
Let $\hilb  V$ be a Hilbert space with $\dim(\hilb V)=d$ finite and let $\ket{i}$ index a basis for $\hilb  V$, such that $\braket{i}{j}=\delta_{ij}$, where $\delta_{ij}$ is Kronecker's delta.  Consider the vectors $\ket{\phi},\ket{\psi}\in \hilb V$ and some $P=\sum_{n=1}^N\ket{n}\bra{n}$ where all $\ket{n}\in\{\ket{i}\}$, and the index $n$ ranges over at most $d$ vectors.  
\begin{enumerate}
 \item[(i)] Show that $P^2=P$ and hence that $P$ is a projector.  Show that $U=-2\sum_n\ket{n}\bra{n}+\eye$ is self-adjoint and unitary.
  \item[(ii)] Give values for the matrix trace and determinant of $U$.  
 \item [(iii)] Show that $(1-\sum_n\ket{n}\bra{n})$ and $(\sum_n\ket{n}\bra{n})$ project onto eigenspaces of $U$, find the corresponding eigenvalues and the maximum dimension of the eigenspaces.   Show that eigenvectors $\ket{\phi}$ in the $+1$ and $-1$ subspaces satisfy $P\ket{\phi} = 0$ and $P\ket{\phi}=\ket{\phi}$, respectively.   
 \item[(iv)] Hence, using these results or otherwise construct an invertible map between projectors and self-adjoint unitary maps.  
\end{enumerate}
\end{myproblem} 

\begin{myproblem}[Tensor products, Density operators, Singular values and purification]
Let $\psi = \ket{001}+\ket{010}+\ket{100}$ be a state in $\hilb H_1\otimes\hilb H_2$ with $\dim(\hilb H_1)=2$ and $\dim(\hilb H_2)=4$, and let  
\begin{equation}
 V^\dagger = \left(
\begin{array}{cccc}
 0 & 1 & 0 & 0 \\
 \frac{1}{\sqrt{2}} & 0 & 0 & -\frac{1}{\sqrt{2}} \\
 \frac{1}{\sqrt{2}} & 0 & 0 & \frac{1}{\sqrt{2}} \\
 0 & 0 & 1 & 0
\end{array}
\right)
\end{equation}
\begin{enumerate}
 \item[(i)] By writing $\phi = \sum_{ij}C_{ij}\ket{i}\ket{j}$, where $\ket{i}\in\hilb H_1$, $\ket{j}\in\hilb H_2$ are both orthonormal basis, state the values of $i\in\{0,1\},j\in\{0,1,2,3\}$ that correspond to non-zero coefficients of $C_{ij}$ and hence express $\psi$ in the basis $\ket{i},\ket{j}$.    
  \item[(ii)]  Write the 2x4 matrix ${\bf C}=(C_{ij})_{ij}$ and show that ${\bf C}{\bf C}^\dagger$ and ${\bf C}^\dagger {\bf C}$ are (non-normalized) density operators, equivalent to $\rho_1$, $\rho_2$ found by tracing over the systems $\hilb H_1$ and $\hilb H_2$ respectively.  (Here the adjoint $\dagger$ means matrix conjugate transpose.)
 \item [(iii)] From the singular value decomposition, one can write ${\bf C}=U\Sigma V^\dagger$.  For $V$ given above, and $U$ the 2x2 identity matrix, find the 2x4 matrix of singular values $\Sigma$.  
 \item[(iv)] Find purifications for $\rho_1$ and $\rho_2$ (other than $\psi$).  
\end{enumerate}
\end{myproblem} 


\begin{myproblem}[Hamiltonians, evolutions, observables and probabilities] 
Recall that the evolution of a quantum system in a static configuration can be found by solving the eigenvalue equation, $H\ket{\psi_n}=E_n\ket{\psi_n}$, where ${\bf H}$ is the Hamiltonian and $E_n$ is the energy of state $\ket{\psi_n}$ written in terms of $\hbar\omega$, where $\omega$ is angular frequency.  The time-evolution of some initial state $\ket{\phi}$ under ${\bf H}$ is then given as 
\begin{equation}
 \ket{\phi(t)}=\sum_n\exp(-it E_n/\hbar)\braket{\psi_n}{\phi}\ket{\psi_n}
\end{equation}
Let the Hamiltonian for a certain three-level system be given as $$
{\bf H}=\hbar\omega\left(\begin{array}{lll}
1 & 0 & 0\\
0 & 2 & 0\\
0 & 0 & 2
\end{array}\right)
$$ and consider the observables 
$$
{\bf A}=\lambda\left(\begin{array}{lll}
0 & 1 & 0\\
1 & 0 & 0\\
0 & 0 & 2
\end{array}\right)
$$
$$
{\bf B}=\mu\left(\begin{array}{lll}
2 & 0 & 0\\
0 & 0 & 1\\
0 & 1 & 0
\end{array}\right)
$$ for positive real constants $\lambda$ and $\mu$.
\begin{enumerate}
 \item[(i)]  Find a map $P$ that transforms the eigenvectors of ${\bf A}$ (given as $\ket{1}+\ket{2}$, $\ket{1}-\ket{2}$, $\ket{3}$) into the eigenvectors of ${\bf B}$. 
 \item[(ii)]  Suppose the system starts out in the generic state $\ket{\psi(0)}= c_1\ket{1}+c_2\ket{2}+c_3\ket{3}$ where $|c_1|^2+|c_2|^2+|c_3|^2=1$.  Find the expectation values at $t=0$ of ${\bf H}$, ${\bf A}$ and ${\bf B}$.  
 \item[(iii)]  Find the time-dependence of the static configuration and hence find $\ket{\psi(t)}$ under the Hamiltonian ${\bf H}$.  
 \item[(iv)]  Determine the possible measured values of the energy of state $\ket{\psi}$ at time $t$.   Likewise, determine the possible measured values values of $\ket{\psi}$ at time $t$ for the observables ${\bf A}$ and ${\bf B}$.  
\end{enumerate}
\end{myproblem} 

\section{Properties of Pauli Matrices}\label{sec:paulibackground} 
Here we recall essential properties of the Pauli matrices, useful for general knowledge and for working through the details of several calculations.  
\begin{mydefinition}
 Recall from angular momentum theory, the familiar Pauli Matrices.  We let $\sigma_1\equiv\sigma_x$, $\sigma_2\equiv\sigma^y$ and $\sigma_3\equiv\sigma^z$ which satisfy 
 \begin{enumerate}
  \item[(i)] $[\sigma_i,\sigma_j] = 2i\epsilon^{ijk}\sigma_k$
  \item[(ii)] complex conjugation is generated by $\sigma_j$ $\forall w\in \{i,j,k\}$ as $\sigma_j\sigma_{w}^*\sigma_j=-\sigma_w$ for $w\neq j$
  \item[(iii)] $\text{tr}{\sigma_i\sigma_j}=2\delta_{ij}$
 \end{enumerate}
 Note that it is common to change subscripts to superscripts $\sigma_x\equiv\sigma^x$ to distinguish powers of operators $\sigma_x^2$ from operators acting on specific indices $\sigma^x_3$ --- that is, $\sigma_x$ acting on the third qubit and not $\sigma_x$ cubed.  This should be evident from context.
\end{mydefinition}

These familiar operators from quantum mechanics form what is called a Geometric Algebra (a.k.a. Clifford Algebra). Consider $\{\sigma^l_i\}$ as a basis for a real left and right distributive vector space, such that
\begin{equation}\label{eqn:geometric1}
\sigma_x^2=\sigma_y^2=\sigma_z^2=\eye=-i\sigma_x\sigma_y\sigma_z
\end{equation}
Then consider the product
\begin{equation}\label{eqn:geoprod}
 \sigma_i\sigma_j = \delta_{ij}\eye + i\epsilon^{ijk}\sigma_k~~~\text{(Geometric product of vectors)}.
\end{equation}
It is clear that for $i\neq j$
\begin{equation}\label{eqn:vanish}
\{\sigma_i^l,\sigma_j^l\}=0
\end{equation} 

meaning that the vectors anti-commute viz.
\begin{equation}\label{eqn:anti}
\sigma_i^l\sigma_j^l=-\sigma_j^l\sigma_i^l.
\end{equation} 
We also note that 
\begin{equation} \label{eqn:eyepauli}
\{\sigma^i,\sigma^j\}=2\delta_{ij}\eye.
\end{equation} 

\begin{myproblem}
 Verify Equations~\eqref{eqn:geoprod}, \eqref{eqn:vanish}, \eqref{eqn:anti} and \eqref{eqn:eyepauli}. 
\end{myproblem}

Single qubit density operators can be expanded in terms of a dot product of a polarisation vector $\underline{P} :=(p_1,p_2,p_3)$, $\forall i, p_i \in \mathbb{R}$, and a sigma vector $\underline{\sigma}:= (\sigma_1, \sigma_2,\sigma_3)$ as
\begin{equation}
\rho = \frac{1}{2}\eye + \underline{\sigma}.\underline{P} =\frac{1}{2}\eye +  p_i\sigma^i = p_1\sigma^1 + p_2\sigma^2 + p_3\sigma^3. 
\end{equation}  
Clearly the vectors $\underline{P}$ are in the vector space $\mathbb{R}^3$.  We can elevate this vector space to a Hilbert space by defining an inner product between vectors --- that is a map $(-,-)$ taking two elements from the vector space (in this case Hamiltonians on $\mathbb{C}^2$) and producing a scalar in the underlining field $\C$.
\begin{equation*}
 (-,-):(\C^2\rightarrow\C^2)\times(\C^2\rightarrow\C^2)\rightarrow \C
\end{equation*}
\begin{equation}
(\underline{\sigma}.\underline{A}, \underline{\sigma}.\underline{B})\mapsto Tr[(\underline{\sigma}.\underline{A}).(\underline{\sigma}.\underline{B})] = \underline{A}.\underline{B}
\end{equation}

\begin{myproblem}%[Product of vectors] 
 Verify that straight forward calculation also yields
\begin{equation}
(\underline{\sigma}.\underline{A},\underline{\sigma}.\underline{B})=A_iB_i + i\epsilon_{ijk}\sigma^k = \underline{A}.\underline{B} + i\underline{\sigma}(\underline{A}\wedge \underline{B}).
\end{equation}
\end{myproblem}

\begin{myproblem}[Eigenvalues] 
 Verify, by using the fact that for $\underline{A}=\underline{B}$ the cross product vanishes or otherwise, that the eigenvalues of $(\underline{A}.\underline{\sigma})$ are $\pm|\underline{A}|$, where both roots necessarily appear as $\underline{A}.\underline{\sigma}$ is traceless. 
\end{myproblem}
%\section*{Problem III. Reminder of quantum circuits, symmetry and eigenstates}

\begin{myproblem}[Further Exercises on Pauli Matricies] 
\begin{enumerate}
 \item[(i)] Let $\underline{P}.\underline{\sigma} := p_0 X + p_1 Y + p_2 Z$ where $|P|=1$ and show that $\exp(-i\frac{\theta}{2}\underline{P}.\underline{\sigma})=\eye \cos(\theta/2)-i(\underline{P}.\underline{\sigma})\sin(\theta/2)$ and find the values of $\theta$, $\underline{P}$ to recover the Hadamard gate, up to a phase factor.  

\item[(ii)] Find the time of the evolution of the Hamiltonian $\ket{11}\bra{11}$ to create a {\sf CZ}-gate, then write down a quantum circuit in terms of {\sf H}  and {\sf CZ} to create a {\sf CNOT}-gate.  What are the input states needed to use the {\sf CNOT}-gate to prepare the singlet state $\ket{\Psi^-}=\ket{01}-\ket{10}$?  

\item[(iii)] Show that the SWAP operator $\frac{1}{2}(\eye + \underline{\sigma}_A\cdot\underline{\sigma}_B)$ permutes the values of bits $A$ and $B$ as 
  \begin{equation}
   \text{SWAP} \ket{i_A}\ket{i_B} = \ket{i_B}\ket{i_A}
  \end{equation}
  where the notation $ \underline{\sigma}_A\cdot\underline{\sigma}_B$ is typically said to stand for the scalar and tensor product. 

\item[(iv)] In the computational basis, express the general form of a two-qubit symmetric eigenstate of the SWAP operator and count the real degrees of freedom.  Repeat this for anti-symmetric eigenstates (e.g. SWAP$\ket{\psi}=-\ket{\psi}$).  
%  \item[(vi)] Express the SWAP operator as a composition of operators of the form
%  \begin{equation}
%  \eta := \sum_i \ket{i}\otimes \ket{i}
% \end{equation}
% \begin{equation}
%  \epsilon := \sum_i \bra{i}\otimes \bra{i}
% \end{equation}
\item[(v)] Using the notation from (iii) above, find a value for $q$ to show that the two-site quantum Heisenberg model $J\underline{\sigma}_1\cdot \underline{\sigma}_2$ can be written as $\frac{J}{2}\left((\underline{\sigma}_1+\underline{\sigma}_2)^2-q\eye\right)$ and show that $\ket{\Psi^\pm}=\ket{01}\pm\ket{10}$ are energy eigenstates.  
\end{enumerate}
\end{myproblem}

==> abstract.tex <==



% 4.1.1. application (stating the applicant’s agreement to use the dissertation in accordance of this Regulation)
% 4.1.2. copy of the document confirming the recognition of education/qualification on the territory of Russian Federation (in other words apostille).
% 4.1.3. copy of PhD diploma + apostille
% 4.1.5. the feedback from scientific advisor (if there is any)
% 4.1.6. no less than two positive feedbacks from specialists, who work on the same thematic but have a higher degree than applicant.
% 4.1.7. the conclusion from the organisation where the approbation of dissertation was held.
% 4.1.8. 9 paper copies of dissertation and in electronic format.
% 4.1.9. the avtoreferat of dissertation in electronic format.
 
% Documents пп. 4.1.1, 4.1.5, 4.1.6, 4.1.7, 4.1.8, 4.1.9 could be in English or Russian languages. Documents пп. 4.1.2, 4.1.3, 4.1.4 are in Russian language or in English language but with the t




\chapter{Extended Thesis Abstract} 

% \section{Classification data}

% \begin{enumerate}
%     \item {\bf Thesis title.} ``On the Theory of Modern Quantum Algorithms''
%     \item {\bf Thesis author.} Jacob Daniel Biamonte, DPhil (Oxon.)\\
% % Associate Professor \\
% % Head of Skoltech’s Laboratory for Quantum Information Processing \\
% % Skolkovo Institute of Science and Technology\\
% % 3 Nobel Street\\
% % Moscow Russia 143026\\


% \item {\bf Subject classification.} Theoretical Physics 01.04.02
% \end{enumerate}

 
\section{Institution of the author}
 
The thesis was written at the Skolkovo Institute of Science and Technology in the years 2018, 2019 and 2020.  The thesis contents are based on research and teaching conducted from 2017 to 2020 in Moscow at the Skolkovo Institute of Science and Technology.  Other aspects (including explanatory approaches) were developed in various places throughout the authors career.
 
\section{Degree advisor(s) and consultant(s)}  
 
\noindent {\bf Sergey N.~Filippov, PhD} \\ 
Associate Professor\\
Head of the Laboratory of Quantum Information Theory \\
Moscow Institute of Physics and Technology \\ 
% Dolgoprudny, Moscow 141701\\
% Russian Federation \\

 
 
\section{Official opponents} 



\noindent {\bf Vladimir Korepin, PhD, DSc} \\ 
Professor \\ 
C.~N.~Yang Institute of Theoretical Physics \\
Stony Brook University \\
% United States \\

\noindent {\bf Alexander Pechen, PhD, DSc} \\ 
Professor \\ 
Steklov Institute, Russian Academy of Sciences\\
Gubkin Street 8, Moscow, 119991, Russian Federation \\

 
\noindent {\bf Walter Pogosov, PhD, DSc} \\ 
Head of the Laboratory of Physics of Micro- and Nanostructures \\ 
Dukhov Research Institute of Automatics \\ 
Russian State Atomic Energy Corporation (Rosatom) \\
%  Sushevskaya 22 Moscow 127055 \\
%  Russian Federation \\






\noindent \textcolor[rgb]{1,0,0}{\bf{[to be continued]}}
 
\section{Leading host organization} 
\noindent International Center for Quantum Optics and Quantum Technologies\footnote{Международный центр квантовой оптики и квантовых технологи} \\ 
\noindent The Russian Quantum Center (RQC) \\
% Novaya 100 Skolkovo\\
% Moscow 143025 \\
% Russian Federation \\ 

% \noindent {Host organization contact}. 
% Alexey Fedorov, PhD \\ 


\section{Relevant dates and abstracting} 
 
\noindent The defense will take place on \textcolor[rgb]{1,0,0}{\bf{[date]}} at the meeting of the dissertation council \textcolor[rgb]{1,0,0}{\bf{[council numbers here]}} in \textcolor[rgb]{1,0,0}{\bf{[address]}}. \\ 
 
In addition to standard circulation by requirement of the Russian Federation rules of higher education, the author confirms that the dissertation has been or will be deposited in the following libraries:
\begin{enumerate}
    \item The library of the Skolkovo Institute of Science and Technology
    \item The library of the Moscow Institute of Physics and Technology
    \item The library of Wolfson College of the University of Oxford\\ Linton Rd, Oxford OX2 6UD, United Kingdom\\
\end{enumerate}

\noindent The dissertation can also be found freely online at:
 \begin{enumerate}
     \item The arXiv preprint server.\footnote{URL. arXiv:TODO}
     \item The overleaf online editor with viewable \LaTeX~source.\footnote{URL.  \url{https://www.overleaf.com/read/xtxxtyygfzjg}} \\
 \end{enumerate} 
 
 \noindent Abstract and thesis sent to official opponents for review on or before 18 May 2020. \\ 
 
 \noindent Abstract and thesis sent to leading host organization for review on or before 18 May 2020. \\ 

\noindent Abstract and thesis sent to dissertation council for review on \textcolor[rgb]{1,0,0}{\bf{[date]}}.\\ 
 
\section{Scientific Secretary of the Dissertation Council \textcolor[rgb]{1,0,0}{[council numbers here]} signature and stamp} 
 
\noindent \begin{tabular}{@{}p{.5in}p{4in}@{}}
Signed:~~ & \hrulefill \\ 
\end{tabular} 
\noindent \\ Ostanina Valentina Olegovna, Engineer \\ 
Scientific Secretary of the Dissertation Council \\
Laboratory of Multimedia Systems and Technologies \\
Moscow Institute of Physics and Technology \\
% Dolgoprudny, Moscow 141701\\
% Russian Federation \\



% \\
% & Ostanina Valentina Olegovna, Engineer \\
% & Scientific Secretary of the Dissertation Council\\
% & Laboratory of Multimedia Systems and Technologies \\
% & Moscow Institute of Physics and Technology \\
% & Dolgoprudny, Moscow 141701\\
% & Russian Federation \\


\section{Technical summary}
 
%{\bf Why is this subject worth studying?} 

Recent developments in quantum information processing have fostered a global research effort to understand and develop  applications for noisy real-world quantum information processors (often called NISQ).\footnote{Noisy Intermediate-Scale Quantum (NISQ) \cite{2018arXiv180100862P}.}  Unlike traditional textbook quantum algorithms, quantum algorithms executed on NISQ devices operate in the presence of systematic and random errors.  Experimental developments have lead to a novel utilitarian means of quantum computation enabled by an iterative classical-to-quantum feedback process called, variational quantum computation.  Variational quantum computation arrives  after ample progress in quantum assisted a.k.a.~quantum accelerated annealing.  While not a general purpose quantum computer in their current form (though universality is possible with further developments \cite{2004quant.ph..5098A}), quantum annealers have been readily available for several years.  Annealers are already in wide use for research and prototyping purposes.  While the capabilities of modern day annealers are fairly well understood, their universal counterparts are not.  
 
Understanding the scope of applications of NISQ-era devices---such as when and how we might expect a quantum speedup and exactly how to program these new machines---is a subject of rapid development.  As the title implies, {\it Modern Quantum Algorithms}, entails precisely the scope of this thesis. Ideas from Hamiltonian complexity and the theory of ground states of physical and synthetic (emulated) Hamiltonians act as a sort of golden thread, uniting variational computation with a better established theory of ground state computation (available as quantum assisted annealing).  This thesis approaches the topic at this intersection with the idea that it should be readable to graduate students.  
 
While a vast number of open questions still remain, on the positive side, Google has recently demonstrated quantum computational supremacy \cite{Arute2019}.  This however is an adversarial game biased to give the quantum processors an evident advantage. Indeed, the task itself is not practical.  Simply put, it represents an elegant abstraction to show that classical computers suffer to emulate quantum ones, even if the quantum computer is not perfect.  While interesting as a milestone, it is not clear how close this result has placed more useful applications.  The questions one might ask are numerous and painfully under explored. Studying some of these questions is the point of this thesis.  We also conclude with a survey of next steps by listing open problems in \S~\ref{chap:conclusion}. 
 
These questions are no longer isolated to a single small community (as was the case just a few years ago).  The topic of quantum algorithms and quantum applications has rapidly transformed from a small academic theoretical community to one driven by major technology leaders and backed by ample private and public investment.  These questions are of central significance today and recent dedicated programs have been started around the globe devoted to their solution (I've written on this global quest with coauthors here \cite{Biamonte2019,Fedorov_2019}).  This thesis sketches a pathway through these contemporary challenges, providing insights and partial solutions to several areas of growing interest.  Care has been taken to make the thesis readable to graduate students.  Readers are assumed to be familiar with quantum computation at the level of one of the common text books \cite{NC}. 
 


 
% % Цель 
\section{The goal of this dissertation}
 
The objective of this thesis is firstly to present a consistent and general unified framework, which conceptually binds together many of the tools used across contemporary quantum programming.  The unifying focus is on properties of ground states of Hamiltonians: 
\begin{enumerate}
    \item[(i)] Programming ground states is required in adiabatic quantum computation and other models of ground state annealing.
    \item[(ii)] It is also central to physics and chemistry simulation algorithms that are anticipated to be promising future applications on quantum computers.
    \item[(iii)] Finally, the variational model of quantum computation is stated by means of a ground state energy optimisation problem that utilises a classical to quantum feedback loop.
\end{enumerate}
The goal is then very simply stated.  We present a coherent view that connects the core ideas across the areas of (i) ground state and adiabatic quantum computation; (ii) the quantum simulation of ground state properties of physical systems; and (iii) the variational approach to Hamiltonian minimisation. We further do so in a way that we believe will be accessible to readers familiar with a standard text book on the subject, such as \cite{NC}. 
 
% % задачи
\section{Tasks performed to achieve dissertation goals} 
 
To present the most central portions of the theory behind the contemporary applications drive, we have to focus on the underlying principles of the theory of ground states as they arise in practical applications of quantum enhanced algorithms.  To accomplish that goal, while making this thesis coherent and as readable as possible, care was taken to introduce the concepts in a pedagogical order.  The logical starting point is understanding how to program ground states of Ising models.  

The thesis therefore begins by recalling several established results related to programming the ground states of generalised Ising systems.  This presents and builds on my own work \cite{B08, spinlogic2}, as well as the work of others \cite{lucas2014ising}.  The topic naturally extends towards more recent work done in collaboration on the area of  the {\it computational phase transition signature} of 3-{\sf SAT} \cite{2019arXiv190610705P}.  This provides an illustrative connection between computational and physical complexity, stated and defined in the early chapter stepwise.  Therefore, to build the first element of the thesis we must present a comprehensive summary of the results on ground state embeddings as they apply to the Ising model.  At this point, we don't assume any time evolution: we consider static Hamiltonians and Gibbs states and no evolution to such states.  

We next must explain the quantum algorithm called, phase estimation.  We survey phase estimation by comparing the evolution of quantum versus stochastic systems.  This adds time dependence and extends the elements we established in the early chapter.  We then must connect this to the quantum circuit model.  From this vantage point, we then introduce the contemporary variational algorithms (QAOA in particular). 

With these elements established, the thesis then presents the unviersal model of variational quantum computation.  In doing so, the early chapters ideas related to programming diagonal Hamiltonin ground states must be revisited and revised to apply to the non-diagonal case.  After doing that, the final chapter also recalls the more general approach to shape Hamiltonian ground states, based on gadget perturbation theory. 




 
 
 
% % Основные положения выносимые на защиту: 
\section{Main statements defended} 
% % Научная новизна: Scientific novelty. "We did X, which was not done before"

\noindent The early chapter establishes two things. 
\begin{enumerate}
    \item Logic operations (gates) can be faithfully embedded into the low-energy sector of Ising spins \cite{B08, spinlogic2}. (including several implications) 
    
    \item The computational phase transition has a signature in Gibbs sampling \cite{Biamonte2019} and is thus (in principle) detectable with near-term physics based processors. 
\end{enumerate}
The first of these assertions is based on (and defended through) deductive reasoning \cite{B08, spinlogic2} where the second is empirically established \cite{2019arXiv190610705P}.

Next, the thesis establishes several interesting relationships between stochastic and quantum walks on graphs.  These results were published as parts of several collaborations (see the review \cite{2017arXiv170208459B}) and only are briefly summarized herein. 

The graphical tensor calculus, called the ZX calculus sometimes, can be used to recover the Gottesman–Knill theorem (see \cite{stabs}).  In other words, \S~\ref{chap:tensornets} establishes that: 
\begin{enumerate}
    \item[3.] The ZX tensor rewrite system admits a poly-time terminating rewrite sequence establishing the Gottesman–Knill theorem.  To establish this we also prove Theorem \ref{theorem:mstg}. We then state Theorem \ref{theorem:gk}. 
\end{enumerate}
This follows by deduction, thereby formally defending the assertion (3). 

The thesis continues by showing several properties relating Grover search and variational algorithms \cite{2018arXiv180509337M}.  It further develops and partially extends an old factorization method originating from Kitaev (appearing in \cite{KSV02}). Finally, the thesis presents the combinatorial quantum circuit area law \cite{biamonte2018entanglement}, 
\begin{enumerate}
    \item[4.] The combinatorial quantum circuit area law bounds the ebits across any bipartion of qubits acted on by a quantum circuit comprised of local unitaries and CNOT gates.  More formally, \\ 
    
    (Lemma \ref{lemma:cqcal}---\cite{UVQC, biamonte2018entanglement}) 
 Let $c$ be the depth of 2-qubit controlled gates in the $n$-qubit hardware-efficient ansatz.  Then the maximum possible number of ebits across any bipartition is 
    $ E_b = \min \{ \left \lfloor{n/2}\right \rfloor, c \}.$ \\ 

\end{enumerate}
The result is established deductively and thereby defended. The chapter then concludes showing that:
\begin{enumerate}
    \item[5.] An order parameter exists that quantifies problem structure in variational algorithms: this correlates with ansatz depth (meaning there exist problem instances that require high depth ansatz circuits). We call this a ``reachability deficit.”
\end{enumerate}
This result (5), as recently published in \cite{2019arXiv190611259A} is established through a combination of deduction and empirical evidence.  It is evidently formulated in a more systematic fashion than in (5) above.  

We follow the statement (5) with a proof related to the variational model \cite{UVQC}, namely: 
\begin{enumerate}
    \item[6.] The variational model formalizes the iterative classical-to-quantum feedback loop to create a universal model of quantum computation stated in terms of objective function minimization \cite{UVQC}. More formally, we have two main results.\\
    
    (Lemma \ref{thm:tele}) Consider $\prod_l U_l \ket{0}^{\otimes n}$ a $L$-gate quantum circuit preparing state $\ket{\psi}$ on $n$-qubits and containing not more than $\mathcal{O}(\text{poly} \ln n)$ non-Clifford gates. Then there exists a Hamiltonian $\mathcal{H}\geq0$ on $n$-qubits with $\text{poly}(L, n)$ cardinality, a $(L, n)$-independent gap $\Delta$ and non-degenerate ground eigenvector $\propto\prod_l U_l \ket{0}^{\otimes n}$.  In particular, a variational sequence exists causing the Hamiltonian to accept $\ket{\phi}$ viz., $0\leq \bra{\phi}\mathcal{H}\ket{\phi}  < \Delta$ then Theorem \ref{thm:e2overlap} implies stability (Theorem \ref{thm:e2overlap}). \\ 
    
    (Theorem \ref{thm:history})
Consider a quantum circuit of $L$ gates on $n$-qubits producing state $\prod_l U_l \ket{0}^{\otimes n}$.  Then there exists an objective function (Hamiltonian, $\mathcal{H}$) with non-degenerate ground state, cardinality $\mathcal{O}(L^2)$ and spectral gap $\Delta\geq \mathcal{O}(L^{-2})$ acting on $n+\mathcal{O}(\ln L)$ qubits such that acceptance implies efficient preparation of the state $\prod_l U_l \ket{0}^{\otimes n}$.  Moreover, a variational sequence exists causing the objective function to accept.  \\ 

\end{enumerate}
The proof that the variational model of quantum computation is universal \cite{UVQC} is defended formally by deductive reasoning. The proof involves introducing constructions that differ from known results.  The proof strategy goes as follows. 
 \begin{enumerate}
     \item[6.i] Stability theorem (relates expected energy with state-overlap)---Lemma \ref{thm:e2overlap}. 
     \item[6.ii] Telescopes (the backbone construction)---Lemma \ref{thm:tele}
     \item[6.ii.a] Clifford invariance of penalty functions---Lemma \ref{lemma:invariance} 
     \item[6.ii.b] Existence of an accepting sequence   
     \item[6.iii] Modify Feynman-Kitaev construction 
     \item[6.iii.a] Set input with a telescope 
     \item[6.iii.b] Prove existence of a gap---Lemma \ref{lemma:gap} 
     \item[6.iii.c] Prove log qubit clock embedding---Lemma \ref{lemma:logem} 
     \item[6.iii.d] Prove boosting lemma $\rightarrow$ show existence of an accepting sequence (given by the quantum circuit being emulated)---Lemma \ref{lemma:uob}  
 \end{enumerate}
The result (6) assumes a noise free system.  Furthermore, the optimization problem typically encountered in variational quantum computation is avoided as follows.  Though somehow artificial, the circuit being emulated itself provides the control sequence which causes the corresponding objective function to accept.  

Finally, the thesis concludes with an overview of the perturbation theory technique used to interelate Hamiltonian models by showing how to emulate new- and higher order interactions using present Hamiltonian terms \cite{BL08, Cao_2015}. Namely, \S~\ref{chap:gadgets}  contains a proof that 
\begin{enumerate}
    \item[7.] The two-body model Hamiltonian 
$$\mathcal{H} = \sum_{i< j} J_{ij}Z_iZ_j + \sum_{i< j} K_{ij}X_iX_j$$ 
is (i) computationally universal for adiabatic quantum computation and (ii) admits a {\bf QMA}-complete ground state energy decision problem \cite{B08}.
\end{enumerate}

The conclusion (\S~\ref{chap:conclusion}) surveys some contemporary open problems. 


 
\section{Scientific novelty}
 
The primary results defended in this thesis have appeared in peer reviewed journals.  I believe the thesis itself culminates to produce an emergent type of novelty.  Indeed, the thesis has an over arching theme: modern quantum programming is presented in terms of computational properties of ground states.  These concepts have played a central role in my own research.  The broadness of scope to have these concepts all presented together with a unifying purpose has certainly not been done before.  

The main results defended in this thesis are easily seen to be novel.  Perhaps the most novel result is the proof that the variational model is computationally universal.  It combines a vast number of known results, tailors them to specific ends and introduces several new lemmas and theorems to support the development and establishment of the theorem(s).  

% 12:03 
% % Практическая значимость
\section{Practical significance} 

Variational methods represent an attractive approach due to the ease at which these algorithms can be realized experimentally.  Contrary to analog quantum simulation, the variational approach forgoes the requirement of realising the targeted Hamiltonian directly in the laboratory, thus allowing the study of a wider variety of previously intractable target models experimentally (including universal penalty functions \cite{UVQC}). This comes at the cost of increased measurements and classical pre- and postprocessing.

Recent state of the art demonstrations include the following: 
\begin{enumerate}
    \item QAOA.  The Google team has used transmon qubits to show QAOA results for up to 17 qubits with depth-3 ansatz levels \cite{2020arXiv200404197A}.  As the authors \cite{2020arXiv200404197A} scaled the number of qubits to produce their dataplot, we believe that they avoided reachability deficits.  A numerical study that places their findings as a cross section of a larger analysis will show the region of their instances, which appear to be statistically representative.  
    \item VQE (chemistry).  The Google team has used transmon qubits to show a VQE approach to create a Hartree-Fock approximation to the ground state of hydrogen chains using 12 qubits in \cite{2020arXiv200404174A}. Their ansatz was of modified checkerboard form. 
    \item VQE (lattice simulation). Self-verifying variational algorithms as proposed in \cite{2019Natur.569..355K} and elsewhere have vanishing objective functions when the solution is reached.  Such an approach was used in \cite{2019Natur.569..355K} to simulate the ground state of the lattice Schwinger model using 8 qubits realized by trapped ions.
\end{enumerate}

The practical significance of this work is readily justified due to this rapid increase in experimental demonstrations of quantum information processing.  Indeed, there is now a global effort to understand the computational capacity and the scope of applications possible on NISQ-era quantum processors (see the popular summary of the topic \cite{Biamonte2019}). Quantum supremacy has also recently been experimentally demonstrated \cite{Arute2019}, which enables certain variational quantum algorithms \cite{2020arXiv200404197A, 2020arXiv200404174A}.   
 
% % Достоверность результатов: 
\section{The validity of the results confirmed by consistency with prior art} 

Many results in this Habilitation thesis date back several years and appeared in peer reviewed journal articles.  They now make up part of the accepted literature on the various topics.  This includes work on Ising model embeddings, work on stochastic versus quantum walks, developing more general perturbation gadgets as well as results on using phase estimation for quantum simulation.  As this is easily seen, we will focus on the variational model.  While these results are mostly published.  Publication is not always peer review in the general setting.  Indeed, the community accepted and used many of the early findings presented here.  I believe this will also be the case for the recent work on variational algorithms: though not enough time has passed to make that a possibility yet.  

This so-called {\it variational} approach to quantum computation, as introduced partly in \cite{2014NatCo...5E4213P, farhi2014quantum}, was formally proven (in the noise free setting) to represent a universal model of quantum computation by the author of this thesis in \cite{UVQC}.  This extended and built on several known results appearing in the related topic of Hamiltonian complexity theory.  Many recent studies have failed to quantify the number of terms needed in the penalty function to implement a variational algorithm.  We hence define a cardinality measure and quantify the number of Pauli terms in the sigma basis.  This is consistent with past findings but presents a new focus to quantify penalty functions.  

In addition, many studies have presented various penalty functions to illustrate that variational algorithms are capable of various tasks.  A universality proof shows that penalty functions in principle are more general.  This is again consistent with the state of the art.  

Little is known about the ultimate practical capacity of the variational model in practice: present tools are difficult to apply to this new framework. Interesting recent findings include the discovery of barren plateaus \cite{McClean_2018} and (together with coauthors) of reachability deficits \cite{2019arXiv190611259A}, a recent connection between variational algorithms and contextuality has been made in \cite{Kirby_2019}, and novel findings relating barren plateaus to circuit depth appeared in \cite{2020arXiv200100550C}. The finding of reachability defictis showed that existing papers applying QAOA are all too often in a low density subset of the possible problem instances.  Hence, representative examples were not considered, which avoided these deficits.  The result is entirely consistent with the state of the art in the topic.  

As variational quantum algorithms rely on minimization of some cost function, an important finding shows how to evaluate the gradients of said cost function exactly \cite{Mitarai_2018,Schuld_2019}. In addition, less general, though equally interesting work includes studying level-1 QAOA \cite{2019arXiv190507047H} and recent findings related to circuit-parameter concentrations between instance solutions \cite{2019arXiv191008187F}.  The topic is developing rapidly. It is already large enough where a single thesis can not cover all of the developments.  However, the core and central ideas are covered here.  These ideas (as developed by many researchers over many years) have remained central to my research.  The foundations are certainly covered here with the main and essential findings outlined in what I hope is an expository fashion.  


 
 
% %Апробация работы: The main results were presented at these conferences...
% % Личный вклад: 
\section{Presentation of thesis contents} 
 
Contents and results from this thesis were presented by the author to peers at the following scientific events. 

\begin{enumerate}
    \item {\bf Variational Models of Quantum Computation}\\ 
Episode IX, Google Research Series on Quantum Computing \\
Google Poland, Warsaw Poland, 10 October 2019 \\
Invited Research Lecture\footnote{Video URL. \url{https://www.youtube.com/watch?v=P52iqU50NHg}} \\ 
    
    \item {\bf A Universal Model of Variational Quantum Computation}\\
Quantum Machine Learning and Data Analytics Workshop \\
Purdue University, Discovery Park, West Lafayette Indiana \\ United States, September 2019 \\
Invited Research Lecture\footnote{Video URL. \url{https://www.purdue.edu/data-science/quantum-machine-learning/}} \\

\item {\bf Quantum Enhanced Machine Learning} \\ 
Physics Challenges in Machine Learning for Network Science \\
Queen Mary University of London\\
London, United Kingdom, September 2019 \\
Invited Research Lecture\footnote{Video URL. \url{https://www.qmul.ac.uk/maths/news-and-events/events-/physics-challenges-for-machine-learning-and-network-science/}}\\

\item {\bf Quantum Machine Learning for Quantum Simulation}\\
Machine Learning for Quantum Matter \\ 
Nodita, Stockholm, Sweden, August 2019 \\
Invited Research Lecture\footnote{Video URL. \url{https://indico.fysik.su.se/event/5644/}} \\

\item {\bf Recent Results in the Theory of Variational Quantum Computation}\\ 
the 5th International Conference on Quantum Technologies \\
The Russian Quantum Center, Moscow Russia 2019 \\
Invited Research Lecture\footnote{Video URL. \url{http://conference.rqc.ru}} \\

\item {\bf Variational Quantum Computation in Photonics}\\ 
The 28th Annual International Laser Physics Workshop \\
Gyeongju, South Korea\\ 
Invited Research Lecture\\

\item {\bf Trends in Variational Quantum Algorithms}\\
Overview style talk given (multiple times) at 
\begin{enumerate}
    \item Riken Institute (Japan)
    \item NTT laboratories (Tokyo, Japan)
    \item CIIRC Institute (Prague)
\end{enumerate}


\item {\bf Quantum Machine Learning Matrix Product States}\\ 
Keynote talk at the Workshop on Quantum Information\\
Harvard, USA, April 23-24, 2018

\item {\bf Quantum Complex Networks}\\
Keynote Lighting Talk at International school and conference on network science (NetSci) \\
Paris, France 2018
% 1000 + attendees

\end{enumerate}

\section{The author's professional impact short summary}
 
The author is an Associate Professor at the Skolkovo Institute of Physics and Technology and the Head of the Institutes Laboratory for Quantum Information Processing.  

As is part of the Russian standard (at least in recent times), impact summaries are typically quantified with citation counts.  As of May 2020, mine are as follows. 
\begin{enumerate}
    \item ORCHID ID {\url{https://orcid.org/0000-0002-0590-3327}} 
    \item Scholarly entries appearing in ORCHID \hfill 74
    \item Total citations\footnote{Data collected from Google Scholar on May 2020.} \hfill 3,214 
    \item Total citations in prior year (2019) \hfill 798
	\item h-index \hfill 26 
	\item i10-index \hfill 39 
	\item Papers in Web of Science top 1\% highly cited papers index: 3 
	\item Papers in Web of Science top 0.1\% highly cited papers index: 1 
\end{enumerate}
 
 
% % Публикации: 
\section{List of relevant publications} 
 
The author confirms their significant or sole involvement in the design and execution of the research published in the following peer reviewed works. 
 
Furthermore, the author asserts that these publications were not used as part of any other degree. \\

\subsubsection{Selected primary research articles related to the thesis contents}

\begin{enumerate}
    \item {\bf Reachability Deficits in Quantum Approximate Optimization} \\ 
V. Akshay, H. Philathong, M.E.S. Morales, J. Biamonte \\ 
Physical Review Letters 124, 090504 (2020)~\cite{2019arXiv190611259A} \\
    
    \item {\bf Entanglement Scaling in Quantum Advantage Benchmarks} \\
Jacob D. Biamonte, Mauro E.S. Morales and Dax Enshan Koh \\ 
Physical Review A 101, 012349 (2020) \cite{biamonte2018entanglement} \\
    
    \item {\bf Ground State Spin Logic} \\ 
J. D. Whitfield, M. Faccin and J. D. Biamonte \\ 
EPL 99, 57004 (2012)~\cite{spinlogic2}\\
{\it Established the symmetry group of penalty Hamiltonian's representing universal logic gates and further reduced known penalty functions.} \\
    
\item {\bf Realizable Hamiltonians for Universal Adiabatic Quantum Computers}\\ 
Jacob Biamonte and Peter Love \\ 
Physical Review A 78, 012352 (2008) \cite{BL08} \\
{\it Solved a standing open problem.  Proved that the two-body model Hamiltonian 
$$\mathcal{H} = \sum_{i< j} J_{ij}Z_iZ_j + \sum_{i< j} K_{ij}X_iX_j$$ 
is (i) computationally universal for adiabatic quantum computation and (ii) admits a {\bf QMA}-complete ground state energy decision problem. These results remain influential, with the paper receiving its highest yearly citation count to date in 2019. } \\ 

\item {\bf Simulation of Electronic Structure Hamiltonians using Quantum Computers} \\ 
James Whitfield, Jacob Biamonte and Alan Aspuru-Guzik \\ 
Molecular Physics 109, 735 (2011) \cite{WBA11} \\
{\it awarded a Longuet-Higgins Paper Prize} \\ 

\item {\bf Adiabatic Quantum Simulators} \\
Jacob Biamonte, Ville Bergholm, James Whitfield, Joe Fitzsimons and Alan Aspuru-Guzik \\
AIP Advances 1, 022126 (2011) \cite{sim11} \\ 

\item {\bf Tensor Network Methods for Invariant Theory} \\
Jacob Biamonte, Ville Bergholm, and Marco Lanzagorta \\ 
Journal of Physics A: Mathematical and Theoretical 46, 475301 (2013) \cite{2013JPhA...46U5301B} \\ 

\item {\bf Tensor Network Contractions for \#SAT} \\
Jacob Biamonte, Jacob Turner and Jason Morton \\
Journal of Statistical Physics 160, 1389 (2015) \cite{2015JSP...160.1389B} \\
{\it Discovered an algorithm using an axiomatic tensor contraction language showing that counting problems can be solved efficiently when their tensor network expression has at most ${\mathcal O}(\log c)$ {\sf COPY}-tensors and polynomial bounded fan-out.} \\

\item {\bf Hamiltonian Gadgets with Reduced Resource Requirements}\\
with Yudong Cao, Ryan Babbush and Sabre Kais \\
Physical Review A 91, 012315 (2015) \cite{Cao_2015} \\ 

\item {\bf Community Detection in Quantum Complex Networks}\\ 
Mauro Faccin, Piotr Migdał, Tomi Johnson, Ville Bergholm, Jacob Biamonte \\
Physical Review X 4, 041012 (2014) \cite{faccin2014community} \\ 

\item {\bf Degree Distribution in Quantum Walks on Complex Networks}\\ 
with Mauro Faccin, Tomi Johnson, Sabre Kais and Piotr Migdal \\
Physical Review X 3, 041007 (2013) \cite{faccin2013degree} \\ 

\item {\bf Undecidability in Tensor Network States} \\
Jason Morton and Jacob Biamonte \\ 
Physical Review A Rapid Communications 86, 030301(R) (2012) \cite{PhysRevA.86.030301} \\ 

\item {\bf Algebraically Contractible Topological Tensor Network States}\\
S. J. Denny, J. D. Biamonte, D. Jaksch and S. R. Clark \\
Journal of Physics A: Mathematical and Theoretical 45, 015309 (2012) \cite{2012JPhA...45a5309D} \\ 

\item {\bf Variationally Learning Grover’s Quantum Search Algorithm} \\
Mauro ES Morales, Tim Tlyachev and Jacob Biamonte \\
Physical Review A 98, 062333 (2018) \cite{2018arXiv180509337M} \\ 

\item {\bf Charged String Tensor Networks} \\ 
Jacob Biamonte \\
Proceedings of the National Academy of Sciences {\bf 114}, 2447 (2017)\\
{\it Proved that (i) $|y_+\rangle=|0\rangle+\imath|1\rangle$, (ii, iii) cups and caps, (iv) Hadamard and (v) {\sf COPY} generate any Clifford tensor network.} \\ 

\item {\bf Spectral Entropies as Information-Theoretic Tools for Complex Network Comparison}\\
Manlio De Domenico and Jacob Biamonte\\
Physical Review X 6, 041062 (2016) \cite{De_Domenico_2016} \\
{\it Defined the first spectral function of a graph satisfying both (i) the definition of an entropy and (ii) subadditivity.} 
\end{enumerate}
 
\section{Books related to the thesis contents}

\begin{enumerate}
    \item {\bf Quantum Tensor Networks: a pathway to modern diagrammatic reasoning}\\ 
Jacob Biamonte \\ 
in review, 178 pages (2020). arXiv:1912.10049  \cite{biamonte2019lectures}\\

\item {\bf Quantum Techniques for Stochastic Mechanics} \\
John C. Baez and Jacob Biamonte \\ 
World Scientific Publishing Co Pte Ltd, 276 pp (2018) \\
ISBN: 978-981-3226-93-7 \cite{2012arXiv1209.3632B}
\end{enumerate}


\subsubsection{Review articles related to the thesis contents}

\begin{enumerate}

\item {\bf Tensor Networks in a Nutshell}\\ 
Jacob Biamonte and Ville Bergholm \\ 
in review (2020) arXiv:1708.00006 \cite{biamonte2017tensor} \\ 


    \item {\bf Complex Networks from Classical to Quantum} \\
Jacob Biamonte, Mauro Faccin and Manlio De Dominico\\
Communications Physics 2, 53 (2019) \cite{2017arXiv170208459B} \\ 

\item {\bf Quantum Machine Learning}\\ 
Jacob Biamonte, Peter Wittek, Nicola Pancotti, Patrick Rebentrost, Nathan Wiebe and Seth Lloyd\\
Nature 549, 195-202 (2017) \cite{2017Natur.549..195B}

\end{enumerate}

\subsubsection{Selected experimental collaborations related to thesis contents}

\begin{enumerate}
\item {\bf Experimental Neural Network Enhanced Quantum Tomography}\\ 
with Adriano Macarone Palmieri, Egor Kovlakov, Federico Bianchi, Dmitry Yudin, Stanislav Straupe and Sergei Kulik \\ 
npj Quantum Information 6:20 (2020) \cite{palmieri2020experimental} \\ 

    \item {\bf Chiral Quantum Walks}\\ 
with Dawei Lu, Jun Li, Hang Li, Tomi H. Johnson, Ville Bergholm, Mauro Faccin, Zoltán Zimborás, Raymond Laflamme, Jonathan Baugh and Seth Lloyd \\
 Physical Review A 93, 042302 (2016) \cite{Lu_2016} \\ 
 
 \item {\bf Quantum Simulation of Helium Hydride Cation in a Solid-State Spin Register}\\ 
with Ya Wang, Florian Dolde, Ryan Babbush, Ville Bergholm, Sen Yang, Ingmar Jakobi, Philipp Neumann, Alan Aspuru-Guzik, James Whitfield and Jorg Wrachtrup \\
ACS Nano 9, 7769 (2015) \cite{Wang2015} \\ 

\item {\bf High Fidelity Spin Entanglement using Optimal Control} \\ 
with Florian Dolde, Ville Bergholm, Ya Wang, Ingmar Jakobi, Sebastien Pezzagna, Jan Meijer, Philipp Neumann, T. Schulte-Herbrüggen and Jorg Wrachtrup \\ 
Nature Communications 5, 3371 (2014) \cite{dolde2014high} \\

\item {\bf Towards Quantum Chemistry on a Quantum Computer}\\ 
with Benjamin Lanyon, James Whitfield, Geoff Gillet, Michael Goggin, Marcelo Almeida, Ben Powell, Marco Barbieri, Alan Aspuru-Guzik and Andrew White \\ 
Nature Chemistry 2, 106 (2009) \cite{Lanyon2010}\\

\item {\bf Sign-and Magnitude-Tunable Coupler for Superconducting Flux Qubits} \\ 
with R Harris, AJ Berkley, MW Johnson, P Bunyk, S Govorkov, MC Thom, S Uchaikin, AB Wilson, J Chung, E Holtham,  A Yu Smirnov, MHS Amin and Alec Maassen van den Brink \\ 
Physical Review Letters 98(17), 177001 (2007) 
\end{enumerate}




\section{Brief chapter descriptions} 

The objective of this thesis has been to pull a thread through the various subjects that have culminated in the modern theory of quantum algorithms.  

At the core of these concepts is the {\sc Local Hamiltonian} problem.  We considered several variants throughout the text.  

The early chapter (\S~\ref{chap:progGS}) presented results which would enable one to sculpt Hamiltonians.  This was done by mapping generalized Ising models between pseudo Boolean functions.  A variety of algebraic tools exist to minimize and manipulate pseudo Boolean and Boolean functions.  Particularly to transform a $k$-body Hamiltonian into a $2$-body one.  My own contributions to programming diagonal ground states appears in \cite{B08} as well as in joint work \cite{spinlogic2, Cao_2015}. Several evident Hamiltonain problems were connected to the theory of computational complexity theory.  

The early chapter also presented some interesting findings \cite{2019arXiv190610705P} which relate physical and computational complexity.  Indeed, we showed that the computational phase transition signature can be physically observed through Gibbs sampling \cite{2019arXiv190610705P}.  This is indeed relevant to current experimental demonstrations and it is the subject of ongoing work to experimentally demonstrate our numerical simulations. 

The next chapter (\S~\ref{chap:qvspc}) presented a comparison between stochastic and quantum mechanics in several capacities.  This comparison is central to my own research as well as ample contemporary studies.  The approach I have taken, with several coauthors, is to establish a comparison inside the language of quantum walks.  Every quantum process admits a quantum walk in the single particle basis, so the model is rather general.  Joint work on this topic centers around \cite{2012arXiv1209.3632B, faccin2013degree, 2017arXiv170208459B, Zimbors2013, Lu_2016, Faccin_2014} subsequently surveyed in \cite{2017arXiv170208459B}. \S~\ref{chap:qvspc} concludes by focusing on a comparison between the quantum and stochastic ground state energy problems. 

Setting the stage for work to come and also presenting a few results, \S~\ref{chap:tensornets} presents tensor networks as well as their relationship with quantum circuits.  The presented results include presenting the minimal generators of stabilizer tensor networks (Theorem \ref{theorem:mstg}).  This proof appeared in my paper \cite{B17}.  The main result of the section was a graphical proof of the Gottesman–Knill Theorem (see Theorem \ref{theorem:gk}).  I am not aware of such a result being previously published though the result is not extremely surprising based on the capacity of the known graphical languages.  

Next \S~\ref{chap:varintro} begins by applying circuits (as a variational ansatz) to approximate optimization problems.  The chapter defines some of the necessary complexity theory background.  Then importantly, the variational model of quantum computation is defined rather precisely, following my work in \cite{UVQC}.  The start of the chapter also follows partially the results from the collaboration published as \cite{2018arXiv180509337M}. 

An old problem of importance is how to realize controlled unitary gates as a sequence of two-body gates.  The chapter presents a factorization that was inspired by work appearing in the book \cite{KSV02}.  With some small but notable improvements, herein we present a competitive method to realize such gates.  We quantify the scaling of the method exactly.  I am unaware of such a result being previously published.  

Towards our goals, we have included a derivation showing that reasonable depth circuits can saturate bipartite entanglement---the depth of these circuits scales with the number of qubits and also depends on the interaction geometry present in a given quantum processor.  This result follows my work \cite{UVQC} as well as the collaboration \cite{biamonte2018entanglement} and establishes a relationship between an objective circuit (to be simulated) and a given ansatz state.

Finally, \S~\ref{chap:varintro} concludes with recalling a fundamental limitation discovered in \cite{2019arXiv190611259A} with coauthors.  The {\sf QAOA} algorithms that exploit variational state preparation to find approximate ground states of Hamiltonians encoding combinatorial optimization problems. In particular we consider the Quantum Aproximate Optimization Algorithm or {\sf QAOA}~\cite{farhi2014quantum}. As a means to study the performance of {\sf QAOA}, we turn to constraint satifiability---a tool with a successful history which was covered in detail in \S~\ref{chap:progGS} (see particularly \S~\ref{sec:cpt}).  Such problems are expressed in terms of $N$ variables and $M$ clauses (or constraints). Interesting, we found that the problems density strongly correlates with the ability of {\sf QAOA} to solve a specific problem instance.  

Going further than \S~\ref{chap:varintro}, next \S~\ref{sec:variational} followed the results in \cite{UVQC} and presented universal penalty functions for variational quantum computation.  The presented penalty functions are formally proven to have a number of desirable qualities.  The objective was to simulate the output of an $L$ gate quantum circuit acting on the $n$-qubit product state $\ket{0}^{\otimes n}$.  We have defined an objective function that when minimized will produce a state close to the desired quantum circuit output. 

We then conclude the presentation of research in \S~\ref{chap:gadgets} by covering several results, many of which are widely used that came primarily out of the work  \cite{BL08, Cao_2015}.  The YY gadget in particular was derived by Yudong Cao.  I attempted the same calculation but stopped after asymmetry caused terms to cancel.  We decided to take the calculation one order further, lead by Yudong. He hence recovered the desired coupling and we worked together to dress the terms and minimize the error.  

In closing, this thesis set out to carve a path through the core area of research related to contemporary quantum programming.  Many of the results presented played their own role in developing the field we have arrived at today, which is dominated by variational algorithms.  Having spent a number of years working on the topic, I found it tantalizing to be able to paint this picture and show some relationships between all of these contemporarily relevant topics.  I hope future readers will indeed find the presentation and explanations, when given, to be of additional value.  There are also a few unpublished results scattered around these pages that might one day become parts of research papers.  

% As I understand right now:

% 1. An order parameter exists that quantifies problem structure: this correlates heavily with ansatz depth (meaning there exist problem instances that require both low and high depth to be able to solve but we need to run an optimization loop to solve them). We call this a “reachability deficit”
% 2. For a long depth circuit, we end up approximating a t-design which implies that there is a vanishing 2nd moment and hence no gradients and hence we can’t train the circuit always
% 3. There further exists examples that can not be trained piecewise (we have such examples)
% 4. The variational model was proven to admit a universal model of quantum computation though the setting was idealised and the quantum circuit itself lifts to a solution of the variational problem to avoid the optimisation loop
% 5. There exists penalty functions with exponential cardinality (number of terms in the Pauli basis) that have vanishing gradients for circuits of depth o(1) 


==> chapter5.tex <==

%\chapter{Low-depth quantum circuits}

\section{Low-depth quantum circuits}

\subsection{A combinatorial quantum circuit area law} 

Our construction of universal variational quantum computation has not considered whether a restricted form of ansatz is capable of universal quantum computation at some arbitrary depth as Lloyd~\cite{2018arXiv181211075L} and others~\cite{morales2019universality} have.  Instead, the objective function to be minimised is defined in terms of the unitary gates arising in the target circuit to be simulated.  What ansatz states are then required to simulate a given target circuit?

This question appears to be difficult and not much is currently known.  In the case of {\bf QAOA} it was recently shown by myself and coauthors that the ability of an ansatz to approximate the ground state energy of a satisfiability instance worsens with increasing problem density (the ratio of constraints to variables) \cite{2019arXiv190611259A}. These related results however do not immediately apply to our interests here.  

Towards our goals, we have included a derivation in the Supplement (see: combinatorial quantum circuit area law) showing that reasonable depth circuits can saturate bipartite entanglement---the depth of these circuits scales with the number of qubits and also depends on the interaction geometry present in a given quantum processor.  This result establishes a first relationship between an objective circuit (to be simulated) and a given ansatz state.  Consider the following.  

An ebit is a unit of entanglement contained in a maximally entangled two-qubit (Bell) state.  A quantum state with $q$ ebits of entanglement (quantified by any entanglement measure) contains the same amount of entanglement (in that measure) as $q$ Bell states.  
\begin{lemma}[Combinatorial Quantum Circuit Area Law---\cite{UVQC}]
 Let $c$ be the depth of 2-qubit controlled gates in the $n$-qubit hardware-efficient ansatz.  Then the maximum possible number of ebits across any bipartition is 
    $$ E_b = \min \{ \left \lfloor{n/2}\right \rfloor, c \}.$$ 
 \end{lemma} 
In a low-depth circuit, the underlying geometry of the processor heavily dictates $c$ above.  For example, for a line of qubits and for a ring, the minimal $c$ required to possibly maximise $E_b$ is $\sim n/2$ and $\sim n/4$ respectively. 
However, in the case of a grid, the minimal depth scales as $\sim \sqrt{2}/2$.  

Hence, if we wish to simulate a quantum algorithm described by a low-depth circuit, having access to a grid architecture could provide an intrinsic advantage.  Specifically, our combinatorial quantum circuit area law establishes that  an objective circuit generating $k< \left \lfloor{n/2}\right \rfloor$ ebits across every bipartition, must be simulated by an ansatz of at least minimal required circuit depth $\sim \sqrt{k}$ on a grid.  

While this does establish a preliminary relationship, the general case remains unclear at the time of writing.  For example, given a quantum circuit with application time $t^\star$ which outputs $\ket{\psi}$, what is the minimal $t(\epsilon)\leq t^\star$ for a control sequence \eqref{eqn:time} to provide an $\epsilon$ close 2-norm approximation to $\ket{\psi}$? 

Here we will consider some properties of the quantum states that are accessible in NISQ era quantum information processing.  Here we provide a bound for the minimal depth circuit (generated from the so called, hardware efficient Ansatz as used in recent experiments \cite{2017Natur.549..242K}) to possibly saturate bipartite entanglement on any bipartition.  Understanding the computational power of these circuits represents a central open question in the field of quantum computation today.  This appendix seeks to quantify contemporary capacities.  We are currently not able to express the success probability as a function of the circuit depth required for an objective function to accept. 

\begin{definition}[Interaction graph]    
Consider the Hamiltonian 
$$ \mathcal{H} = \sum_{ij} J_{ij} A_i A_j + \sum_i b_i B_i  + \sum_i c_i C_i. $$
The support matrix $S$ of $J_{ij}$ is defined to have the entries
 $$ S_{ij} =  [J_{ij}]^0 $$
 and is called the \textit{interaction graph of $\mathcal{H}$}---a symmetric adjacency matrix.
\end{definition} 


\begin{remark} 
The interaction graph induces a space-time quantum circuit defined by a \textit{tiling} on the multiplex from $S$.
\end{remark}

\begin{definition} 
 A \textit{Tiling} is a gate sequence acting on a multiplex network induced by $S$.  
 \end{definition} 
 
 \begin{remark}     An active edge (node) will specify if neighboring edges (nodes) can be active. As a general rule, non-commuting terms must be active on different layers.  
     \begin{enumerate}
        \item Qubits connect network layers by time propagation.
        \item Nodes of $S$ in each layer can be acted on by local gates.
        \item Edges of $S$ in each layer can be acted on by two-qubit gates. 
    \end{enumerate}
 \end{remark} 
   
 As an example, consider the following multiplex network.    
    % \begin{center}
    %     \minipage{0.5\textwidth}
    %     \includegraphics[width=\linewidth]{multiplex.pdf}
    %     \endminipage
    % \end{center}
 \begin{figure}[p]
 
    \begin{center}
        \minipage{0.5\textwidth}
        \includegraphics[width=\linewidth]{multiplex.pdf}
        \endminipage
        \minipage{0.01\textwidth}
        \begin{tikzpicture}[scale=5, axis/.style={very thick, ->, >=stealth'}]
            \draw[axis] (0,-0.1) -- (0,1.1) node(yline)[above] {$t$};
        \end{tikzpicture}
        \endminipage
    \end{center}
    % \captionof{labelformat=empty}
    \captionof{figure}{Five qubits evolve as time goes up on the page.  At $t=0$, commuting interaction terms (red edges) are applied between the qubits.  At $t=1$ local gates (red nodes) are applied to each of the qubits. }
 \end{figure}
    
    In the bottom layer a sequence of red edges correspond to the application of two-body gates.  In the next layer, the red (active) notes correspond to local rotation gates being applied to all the qubits. Finally, in the top layer the commuting two-body gates are applied.  The blue vertical edges represent time passing (going up on the page).  The hardware-efficient ansatz is exactly such a tiling.  
    
In terms of example circuits, we typically will be given a short repetitive sequence.  For example, here we consider qubits interacting on a ring.  A layer of local gates followed by a layer of two-body gates is as follows.     
    
    % \begin{equation*}
    %     \Qcircuit @C=.75em @R=.75em {
    %         & \gate{U_1} & \qw & \qw & \ctrl{1}   & \qw        & \qw        & \gate{R_Y} & \qw \\
    %         & \gate{U_2} & \qw & \qw & \gate{R_Y} & \ctrl{1}   & \qw        & \qw        & \qw \\
    %         & \gate{U_3} & \qw & \qw & \qw        & \gate{R_Y} & \ctrl{1}   & \qw        & \qw \\
    %         & \gate{U_4} & \qw & \qw & \qw        & \qw        & \gate{R_Y} & \ctrl{-3}  & \qw \\
    %     }
    % \end{equation*}
    \begin{equation*}
        \Qcircuit @C=.75em @R=.75em {
            & \gate{U} & \qw & \qw & \ctrl{1}   & \qw        & \qw & \qw    & \qw & \qw        & \gate{R_Y} & \qw \\
            & \gate{U} & \qw & \qw & \gate{R_Y} & \ctrl{1}   & \qw & \qw    & \qw & \qw        & \qw        & \qw \\
            & \gate{U} & \qw & \qw & \qw        & \gate{R_Y} & \qw & \qw    & \qw & \ctrl{2}   & \qw        & \qw \\
            &          &     &     &            &            &     & \ddots &     &            &            &     \\
            & \gate{U} & \qw & \qw & \qw        & \qw        & \qw & \qw    & \qw & \gate{R_Y} & \ctrl{-4}  & \qw \\
        }
    \end{equation*}
    
    \bigskip
    
Where the local gates, $U$ are arbitrary and the two-body gates are controlled $Y$ rotations.  What is the maximal bipartite entanglement that such a circuit can generate when acting on a product state? 

To understand this question, let us consider a pure $n$-qubit state $\ket{\psi}$. 

\begin{definition} 
Bipartite rank is the Schmidt number (the number of non-zero singular values) across any reduced bipartite density state from $\ket{\psi}$ (i.e.~$\lfloor n/2 \rfloor$ qubits).  
\end{definition} 

\begin{remark} 
Rank provides an upper-bound on the bipartite entanglement that a quantum state can support---a rank-$k$ state has at most $\log_2(k)$ ebits of entanglement. 
\end{remark} 

\begin{definition}
An ebit is a unit of entanglement contained in a maximally entangled two-qubit (Bell) state. 
\end{definition} 

\begin{remark} 
A quantum state with $q$ ebits of entanglement (quantified by any entanglement measure) contains the same amount of entanglement (in that measure) as $q$ Bell states. 
\end{remark} 

\begin{remark} 
If a task requires $r$ ebits, it can be done with $r$ or more Bell states, but not with fewer.  Maximally entangled states in $\mathbb{C}^d\otimes \mathbb{C}^d$ have $\log_2(d)$ ebits of entanglement. 
\end{remark} 

Now we arrive at what we call a {\it quantum circuit combinatorial area law}.  It is the minimal depth circuit that possibly could saturate the bipartite entanglement with respect to any bipartition. 

\begin{lemma}
 Let $c$ be the depth of 2-qubit controlled gates in the $n$-qubit hardware-efficient ansatz.  Then the maximum possible number of ebits across any bipartition is 
    $$ \min \{ \left \lfloor{n/2}\right \rfloor, c \}.$$ 
 \end{lemma} 
 
%  \begin{example}[Combinatorial quantum circuit area law] 
%     Minimal possible $c$ saturating for specific graph. 
    
%     \begin{center}
%         \minipage{0.3\textwidth}
%         \includegraphics[width=0.9\linewidth]{line.pdf}
%         \endminipage
%         $\qquad \quad c \sim n/2$
        
%         \minipage{0.3\textwidth}
%         \includegraphics[width=.9\linewidth]{ring.pdf}
%         \endminipage
%         $\qquad \quad c \sim n/4$
    
%         \minipage{0.35\textwidth}
%         \includegraphics[width=\linewidth]{grid.pdf}
%         \endminipage
%         $\qquad \quad c \sim \sqrt{n}/2$
%     \end{center}
% \end{example} 
 \begin{remark}[Combinatorial Quantum Circuit Area Law] 
    Minimal possible $c$ saturating specific graphs are given in Table \ref{tab:cqcal}. 
 \end{remark}

\begin{table}[p]
  \centering
  \begin{tabular}{p{1.95cm}|c|c|c}
     & line & ring & gird \\
    \hline    \hline
    interaction geometry
    &
    \begin{minipage}{.25\textwidth}
      \includegraphics[width=1.\linewidth]{line.pdf}
    \end{minipage}
    &
    \begin{minipage}{.25\textwidth}
      \includegraphics[width=1.\linewidth]{ring.pdf}
    \end{minipage}
    &
    \begin{minipage}{.25\textwidth}
      \includegraphics[width=1.\linewidth]{grid.pdf}
    \end{minipage}
    \\
    \hline
    saturating depth & $c \sim n/2$ & $c \sim n/4$ & $c \sim \sqrt{n}/2$

  \end{tabular}
  \caption{Minimal possible circuit depth $c$ possibly saturating bipartite entanglement with respect to different interaction geometries.}\label{tab:cqcal}
\end{table}



\section{Reachability Deficits}



In this section we explore a fundamental limitation discovered in \cite{2019arXiv190611259A} with coauthors.  The {\bf QAOA} algorithms that exploit variational state preparation to find approximate ground states of Hamiltonians encoding combinatorial optimization problems. 

In particular we consider the Quantum Aproximate Optimization Algorithm or {\bf QAOA}~\cite{farhi2014quantum}. As a means to study the performance of {\bf QAOA}, we turn to constraint satifiability---a tool with a successful history which was covered in detail in \S~\ref{chap:progGS} (see particularly \S~\ref{sec:cpt}).  Such problems are expressed in terms of $N$ variables and $M$ clauses (or constraints). 

\begin{remark}
Recall from \S~\ref{sec:cpt}, the density of such problem instances is the clause to variable ratio, the clause density $\alpha = M/N$. $k$-{\sf SAT} clauses are randomly generated to form instances by uniformly selecting unique $k$-tupels from the union of a variable set (cardinality $n>k$) and its element wise negation.  We consider random instances of the {\sf NP}-complete decision problem, $3$-{\sf SAT}. 
\end{remark}


{\bf QAOA} aims to approximate solutions to optimization version of this problem.  Here we consider MAX-3-{\sf SAT} which is {\sf NP}-Hard for exact solutions and {\sf APX}-complete for approximations beyond a certain ratio \cite{haastad2001some}. In these settings, the algorithm's limiting performance exhibits strong dependence on the problem density. As discovered in \cite{2019arXiv190611259A}. 

Let \textit{N} be the number of variables in a {\sf SAT} instance with $M$ clauses. MAX-{\sf SAT} solutions are the Boolean strings $\bm{\omega} = \omega_1, \omega_2, \omega_3, ..., \omega_N$ that violate the least number of clauses. Techniques discussed in \S~\ref{chap:progGS} map {\sf SAT} instances into Hamiltonians,  

\begin{equation}\label{3sathamiltonian}
    \mathcal{H}_{\text{SAT}} = \sum_{l=1}^{M}\mathcal{P}(l),
\end{equation}

\noindent where $\mathcal{P}(l)$ are rank-1 projectors acting on the $l^{th}$ clause. It is easy to verify that the ground state energy of $\mathcal{H}_{\text{SAT}}$ is representative of the minimum number of violated clauses. 

The variational state generated by {\bf QAOA} can be described as running a \textit{p}-depth quantum circuit on the state $\ket{+}^{\otimes{n}}$,
\begin{equation}\label{qaoa equation}
    \ket{\psi(\boldsymbol{\gamma},\boldsymbol{\beta})}=\prod_{i=1}^{p} \mathcal{U}(\gamma_{i},\beta_{i})\ket{+}^{\otimes{n}},
    \end{equation} 
    where
\begin{equation}\label{driverandproblem}
    \mathcal{U}(\gamma_{k},\beta_{k})=\exp{-\imath \beta_{k}\mathcal{H}_{x}} \cdot \exp{-\imath \gamma_{k}\mathcal{V}}.
\end{equation}

In order to approximate solutions of MAX-{\sf SAT}, {\bf QAOA} with standard settings, $\mathcal{H}_x=\sum_{i}\sigma_{x}^{(i)}$ and $\mathcal{V} = \mathcal{H}_{\text{SAT}}$, is used to calculate the energy approximation $E_{g}^{\text{QAOA}}$, where

\begin{equation}\label{qaoaoptimization}
    E_{g}^{\text{QAOA}} =  \min_{\boldsymbol{\gamma},\boldsymbol{\beta}} \bra{\psi(\boldsymbol{\gamma},\boldsymbol{\beta})}\mathcal{H}_{\text{SAT}}\ket{\psi(\boldsymbol{\gamma},\boldsymbol{\beta})}.
\end{equation} 


We numerically studied $f = E_{g}^{\text{QAOA}} - \min(\mathcal{V})$ as a function of clause density $\alpha$, for a \textit{p}-depth {\bf QAOA} circuit on randomly generated $3$-{\sf SAT} instances (see Figure~\ref{fig:qaoareachability}). Although increased depth versions achieve better approximations, the limiting performance exhibits a non-trivial dependence on the problem density. Based on this finding we formulate the following:   
 
\begin{definition}
 Let $\ket{\psi}$, be the ansatz states generated from a \textit{p}--depth {\bf QAOA} circuit as shown in \eqref{qaoa equation}. Then 
\begin{equation}\label{eqn:reachabilitydef}
    f = \min_{\psi \subset \mathcal{H}} \bra{\psi}\mathcal{V}\ket{\psi} - \min_{\phi \in \mathcal{H}} \bra{\phi}\mathcal{V}\ket{\phi},
\end{equation}
characterises the limiting performance of {\bf QAOA}. The R.H.S.~of equation \eqref{eqn:reachabilitydef} can be expressed as a function, $f(p,\alpha,n)$.
\end{definition}


\begin{proposition}[Reachability Deficit \cite{2019arXiv190611259A}]
For $p \in \mathbb{N}$ and fixed problem size, $\exists$ $ \alpha > \alpha_c$ such that $f$ from \eqref{eqn:reachabilitydef} is non-vanishing. This is a reachability deficit.
\end{proposition}



\begin{figure}[p]
  \centering 
  \includegraphics[width=0.67\textwidth]{3SATqaoastandard.pdf}
  \caption{$f = E_{g}^{\text{QAOA}} - \min(\mathcal{H}_{SAT})$ vs clause density for $3$-{\sf SAT} for differing {\bf QAOA} depths. Squares show the average value obtained over 100 randomly generated instances for $n=6$ with error bars indicating the standard error of mean. Figure taken from \cite{2019arXiv190611259A}.  }
\label{fig:qaoareachability}
\end{figure}
\vspace{10pt}
\noindent





==> common/characteristic.tex <==
{\actuality} Обзор, введение в тему, обозначение места данной работы в
мировых исследованиях и~т.\:п., можно использовать ссылки на другие
работы~\cite{Gosele1999161} (если их нет, то в автореферате
автоматически пропадёт раздел <<Список литературы>>). Внимание! Ссылки
на другие работы в разделе общей характеристики работы можно
использовать только при использовании \verb!biblatex! (из-за технических
ограничений \verb!bibtex8!. Это связано с тем, что одна и та же
характеристика используются и в тексте диссертации, и в
автореферате. В последнем, согласно ГОСТ, должен присутствовать список
работ автора по теме диссертации, а \verb!bibtex8! не умеет выводить в одном
файле два списка литературы).

 \aim\ данной работы является \ldots

Для~достижения поставленной цели необходимо было решить следующие {\tasks}:
\begin{enumerate}
  \item Исследовать, разработать, вычислить и~т.\:д. и~т.\:п.
  \item Исследовать, разработать, вычислить и~т.\:д. и~т.\:п.
  \item Исследовать, разработать, вычислить и~т.\:д. и~т.\:п.
  \item Исследовать, разработать, вычислить и~т.\:д. и~т.\:п.
\end{enumerate}

\defpositions
\begin{enumerate}
  \item Первое положение
  \item Второе положение
  \item Третье положение
  \item Четвертое положение
\end{enumerate}

\novelty
\begin{enumerate}
  \item Впервые \ldots
  \item Впервые \ldots
  \item Было выполнено оригинальное исследование \ldots
\end{enumerate}

\influence\ \ldots

\reliability\ полученных результатов обеспечивается \ldots \ Результаты находятся в соответствии с результатами, полученными другими авторами.

\probation\
Основные результаты работы докладывались~на:
перечисление основных конференций, симпозиумов и~т.\:п.

\contribution\ Автор принимал активное участие \ldots

%\publications\ Основные результаты по теме диссертации изложены в ХХ печатных изданиях~\cite{Sokolov,Gaidaenko,Lermontov,Management},
%Х из которых изданы в журналах, рекомендованных ВАК~\cite{Sokolov,Gaidaenko}, 
%ХХ --- в тезисах докладов~\cite{Lermontov,Management}.

\ifthenelse{\equal{\thebibliosel}{0}}{% Встроенная реализация с загрузкой файла через движок bibtex8
    \publications\ Основные результаты по теме диссертации изложены в XX печатных изданиях, 
    X из которых изданы в журналах, рекомендованных ВАК, 
    X "--- в тезисах докладов.%
}{% Реализация пакетом biblatex через движок biber
%Сделана отдельная секция, чтобы не отображались в списке цитированных материалов
    \begin{refsection}%
        \printbibliography[heading=countauthornotvak, env=countauthornotvak, keyword=biblioauthornotvak, section=1]%
        \printbibliography[heading=countauthorvak, env=countauthorvak, keyword=biblioauthorvak, section=1]%
        \printbibliography[heading=countauthorconf, env=countauthorconf, keyword=biblioauthorconf, section=1]%
        \printbibliography[heading=countauthor, env=countauthor, keyword=biblioauthor, section=1]%
        \publications\ Основные результаты по теме диссертации изложены в \arabic{citeauthor} печатных изданиях\nocite{bib1,bib2}, 
        \arabic{citeauthorvak} из которых изданы в журналах, рекомендованных ВАК\nocite{vakbib1,vakbib2}, 
        \arabic{citeauthorconf} "--- в тезисах докладов\nocite{confbib1,confbib2}.
    \end{refsection}
}
При использовании пакета \verb!biblatex! для автоматического подсчёта
количества публикаций автора по теме диссертации, необходимо
их здесь перечислить с использованием команды \verb!\nocite!.
    



==> common/concl.tex <==
%% Согласно ГОСТ Р 7.0.11-2011:
%% 5.3.3 В заключении диссертации излагают итоги выполненного исследования, рекомендации, перспективы дальнейшей разработки темы.
%% 9.2.3 В заключении автореферата диссертации излагают итоги данного исследования, рекомендации и перспективы дальнейшей разработки темы.
\begin{enumerate}
  \item На основе анализа \ldots
  \item Численные исследования показали, что \ldots
  \item Математическое моделирование показало \ldots
  \item Для выполнения поставленных задач был создан \ldots
\end{enumerate}


==> common/renames.tex <==
%%% Переопределение именований %%%
\renewcommand{\alsoname}{see also}
\renewcommand{\seename}{see}
\renewcommand{\headtoname}{вх.}
\renewcommand{\ccname}{исх.}
\renewcommand{\enclname}{вкл.}
\renewcommand{\pagename}{P.}
\renewcommand{\partname}{Part}
\renewcommand{\abstractname}{Аннотация}
\renewcommand{\contentsname}{Contents} % (ГОСТ Р 7.0.11-2011, 4)
\renewcommand{\figurename}{Figure} % (ГОСТ Р 7.0.11-2011, 5.3.9)
\renewcommand{\tablename}{Table} % (ГОСТ Р 7.0.11-2011, 5.3.10)
\renewcommand{\indexname}{Предметный указатель}
\renewcommand{\listfigurename}{List of figures}
\renewcommand{\listtablename}{List of tables}
\renewcommand{\refname}{\fullbibtitle}
\renewcommand{\bibname}{\fullbibtitle}

\renewcommand{\appendixname}{Appendix}
\renewcommand{\chaptername}{Chapter}

% %%% Переопределение именований %%%
% \renewcommand{\alsoname}{см. также}
% \renewcommand{\seename}{см.}
% \renewcommand{\headtoname}{вх.}
% \renewcommand{\ccname}{исх.}
% \renewcommand{\enclname}{вкл.}
% \renewcommand{\pagename}{Стр.}
% \renewcommand{\partname}{Часть}
% \renewcommand{\abstractname}{Аннотация}
% \renewcommand{\contentsname}{Оглавление} % (ГОСТ Р 7.0.11-2011, 4)
% \renewcommand{\figurename}{Рисунок} % (ГОСТ Р 7.0.11-2011, 5.3.9)
% \renewcommand{\tablename}{Таблица} % (ГОСТ Р 7.0.11-2011, 5.3.10)
% \renewcommand{\indexname}{Предметный указатель}
% \renewcommand{\listfigurename}{Список рисунков}
% \renewcommand{\listtablename}{Список таблиц}
% \renewcommand{\refname}{\fullbibtitle}
% \renewcommand{\bibname}{\fullbibtitle}


==> qma.tex <==

%\chapter{Hamiltonian complexity}  

\sec{Hamiltonian Complexity}\label{sec:qma}

What is the simplest Hamiltonians that allow universal adiabatic quantum computation?  For this we turn to the complexity class quantum-Merlin-Arthur (\QMA{}), the quantum analog of \NP{}, and consider the \QMA{}-complete problem k-\LH{}~\cite{KSV02}.  One solves k-\LH{} by determining if there exists an eigenstate with energy above a given value or below another---with a promise that one of these situations is the case---when the system has at most k-local interactions.  A \YES{} instance is shown by providing a witness eigenstate with energy below the lowest promised value.

The problem 5-\LH{} was shown to be \QMA{}-complete by Kitaev~\cite{KSV02}.  To accomplish this, Kitaev modified the autonomous quantum computer proposed by Feynman~\cite{Fey82}.  This modification later inspired a proof of the polynomial equivalence between quantum circuits and adiabatic evolutions by Aharonov et al.~\cite{2004quant.ph..5098A}.  Kempe, Kitaev and Regev subsequently proved \QMA{}-completeness of $2$-\LH{}~\cite{KKR06}.  Oliveira and Terhal then showed that universality remains even when the $2$-local Hamiltonians act on particles in a subgraph of the {\sc 2D} square lattice~\cite{OT06}. Any \QMA{}-complete Hamiltonian may realize universal adiabatic quantum computation, and so these results are also of interest for the implementation of quantum computation.

Since $1$-\LH{} is efficiently solvable, an open question is to determine which combinations of $2$-local interactions allow one to build \QMA{}-complete Hamiltonians.  Furthermore, the problem of finding the minimum set of interactions required to build a universal adiabatic quantum computer is of practical, as well as theoretical, interest: every type of $2$-local interaction requires a separate type of physical interaction.  To address this question we prove the following theorems:


\begin{theorem}[ZZXX Hamiltonian \cite{BL08}]
\emph{The problem \SH{} is \QMA{}-complete, with the ZZXX Hamiltonian given as: }
\begin{eqnarray}\label{eqn:zzxx}
H_{\text{ZZXX}}&=&\sum_{i}h_i\PZi+\sum_{i}\Delta_i\PXi+\\\nonumber
&+&\sum_{<i,j>}J_{ij}\PZi\Zj+\sum_{<i,j>}K_{ij}\PXi\Xj.
\end{eqnarray}
\end{theorem}

\begin{theorem}[ZX Hamiltonian \cite{BL08}]
\emph{The problem \AH{} is \QMA{}-complete, with the ZX Hamiltonian given as}
\begin{eqnarray}\label{eqn:zx}
{H}_{\text{ZX}}&=&\sum_{i}h_i\PZi+\sum_i\Delta_i\PXi+\\\nonumber
&+&\sum_{<i,j>}J_{ij}\PZi\Xj+\sum_{<i,j>}K_{ij}\PXi\Zj.
\end{eqnarray}
\end{theorem}



\section{{\scshape Local Hamiltonian} is {\sf QMA}-complete}

The translation from quantum circuits to adiabatic evolutions began when Kitaev~\cite{KSV02} replaced the time-dependence of gate model quantum algorithms with spatial degrees of freedom using the non-degenerate ground state of a positive semidefinite Hamiltonian:
\begin{eqnarray}\label{eqn:htot}
&&0=H\ket{\psi_{\text{hist}}} = \\
&&(H_{\text{in}}+ H_{\clock}+ H_{\text{clockinit}}+ H_{\text{prop}})\ket{\psi_{\text{hist}}}.\nonumber
\end{eqnarray}
To describe this, let $T$ be the number of gates in the quantum circuit with gate sequence $U_T\cdots U_2U_1$ and let $n$ be the number of logical qubits acted on by the circuit.  Denote the circuit's classical input by $\ket{x}$ and its output by $\ket{\psi_{\text{out}}}$.  The {\em history state} representing the circuit's entire time evolution is:
\begin{eqnarray}
\ket{\psi_{\text{hist}}}&=& \frac{1}{\sqrt{T+1}}\biggl[\ket{x}\otimes\ket{0}^{\otimes T}+U_1\ket{x}\otimes\ket{1}\ket{0}^{\otimes T-1}\nonumber\\
&+&U_2U_1\ket{x}\otimes\ket{11}\ket{0}^{\otimes T-2}\nonumber\\
&+&\ldots\\
&+&U_T\cdots
U_2U_1\ket{x}\otimes\ket{1}^{\otimes T}\biggr],\nonumber
\end{eqnarray}
where we have indexed distinct time steps by a $T$ qubit unary clock.  In the following, tensor product symbols separate operators acting on logical qubits (left) and clock qubits (right).

$H_{\text{in}}$ acts on all $n$ logical qubits and the first clock qubit.  By annihilating time-zero clock states coupled with classical input $x$, $H_{\text{in}}$ ensures that valid input state ($\ket{x}\otimes\ket{0...0}$) is in the low energy eigenspace:
\begin{eqnarray}\label{eqn:Hin}
H_{\text{in}}&=&\sum_{i=1}^n (\openone-\ket{x_i}\bra{x_i})\otimes \ket{0}\bra{0}_1\\
&+&\left(\frac{1}{4}\right)\sum_{i=1}^n(\openone -(-1)^{x_i}\PZi)\otimes(\openone+\Z_1).\nonumber
\end{eqnarray}

$H_{\clock}$ is an operator on clock qubits ensuring that valid unary clock states $\ket{00...0}$, $\ket{10..0}$, $\ket{110..0}$ etc., span the low energy eigenspace:
\begin{eqnarray}\label{eqn:Hclock}
&&H_{\clock}=\sum_{t=1}^{T-1}\ketbra{01}{01}_{(t,t+1)}\\
&&=\frac{1}{4}\left[(T-1)\openone+\Z_1-\Z_T-\sum_{t=1}^{T-1}\Z_t\Z_{(t+1)}\right],\nonumber
\end{eqnarray}
where the superscript $(t,t+1)$ indicates the clock qubits acted on by the projection. This Hamiltonian has a simple physical interpretation as a line of ferromagnetically coupled spins with twisted boundary conditions, so that the ground state is spanned by all states with a single domain wall. The term $H_{\text{clockint}}$ applies a penalty $\ket{1}\bra{1}_{t=1}$ to the first qubit to ensure that the clock is in state $\ket{0}^{\otimes T}-$ at time $t=0$.

$H_{\text{prop}}$ acts both on logical and clock qubits. It ensures that the ground state is the history state corresponding to the given circuit. $H_{\text{prop}}$ is a sum of $T$ terms, $H_{\text{prop}} =  \sum_{t=1}^T H_{{\text{prop}},t}$, where each term checks that the propagation from time $t-1$ to $t$ is correct.  For $2 \leq t \leq T-1$, $H_{{\text{prop}},t}$ is defined as:
\begin{eqnarray}\label{eqn:Hprop1}
H_{{\text{prop}},t}&\bydef&\openone \otimes \ketbra{t-1}{t-1} - U_t\otimes\ketbra{t}{t-1}\nonumber\\
&&~- U_t^\dag \otimes \ketbra{t-1}{t} + \openone \otimes\ketbra{t}{t},
\end{eqnarray}
where operators ${\ketbra{t}{t-1}=\ketbra{110}{100}_{(t-1,t,t+1)}}$ etc., act on clock qubits $t-1$, $t$, and $t+1$ and where the operator $U_t$ is the $t^{th}$ gate in the circuit. For the boundary cases ($t=1,T$), one writes $H_{{\text{prop}},t}$ by omitting a clock qubit ($t-1$ and $t+1$ respectively).

We have now explained all the terms in the Hamiltonian from Eq.~\eqref{eqn:htot}---a key building block used to prove the \QMA{}-completeness of $5$-\LH{}~\cite{KSV02}.  The construction reviewed in the present section was also used in a proof of the polynomial equivalence between quantum circuits and adiabatic evolutions~\cite{2004quant.ph..5098A}.  Which physical systems can implement the Hamiltonian model of computation from Eq.~\eqref{eqn:htot}?  Ideally, we wish to find a simple Hamiltonian that is in principle realizable using current, or near-future technology.  The ground states of many physical systems are real-valued, such as the ground states of the Hamiltonians from Eq.~\eqref{eqn:zzxx} and~\eqref{eqn:zx}.  So a logical first step in our program is to show the \QMA{}-completeness of general real-valued local Hamiltonians.



\subsection{{\scshape Real Hamiltonian} is {\sf QMA}-complete}


One can show that \RFLH{} is already \QMA{}-complete---leaving the proofs in~\cite{KSV02} otherwise intact and changing only the gates used in the circuits.  $H_{\text{in}}$ from~\eqref{eqn:Hin} and $H_{\text{clock}}$ from~\eqref{eqn:Hclock} are already real-valued and at most $2$-local.  Now consider the terms in $H_{\text{prop}}$ from~\eqref{eqn:Hprop1} for the case of {\em self-inverse} elementary gates $U_t=U_t^\dagger$:
\begin{eqnarray}\label{eqn:Hprop}
H_{{\text{prop}},t}&=&\frac{\openone}{4}(\openone-\Z_{(t-1)})(\openone+\Z_{(t+1)})\\
&-&\frac{U}{4}(\openone-\Z_{(t-1)})\X_t(\openone+\Z_{(t+1)})\nonumber
\end{eqnarray}
For the boundary cases ($t=1,T$), define:
\begin{eqnarray}\label{eqn:H1T}
H_{\text{prop,1}} &=& \frac{1}{2}(\openone+\Z_2)-U_1\otimes\frac{1}{2}(\X_1+\X_1\Z_2)\\\nonumber
H_{{\text{prop}},T} &=& \frac{1}{2}(\openone-\Z_{(T-1)})-U_T\otimes\frac{1}{2}(\X_T-\Z_{(T-1)}\X_T).
\end{eqnarray}
The terms from~\eqref{eqn:Hprop} and~\eqref{eqn:H1T} acting on the clock space are already real-valued and at most $3$-local.  As an explicit example of the gates $U_t$, let us define a universal real-valued and self-inverse 2-qubit gate:
\begin{equation*}
R_{ij}(\phi)=\frac{1}{2}(\openone+\PZi)+\frac{1}{2}(\openone-\PZi)\otimes(\sin(\phi)\PXi+ \cos(\phi)\Zj).
\end{equation*}
The gate sequence $R_{ij}(\phi)R_{ij}(\pi/2)$ recovers the universal gate from~\cite{RG02}. This is a continuous set of elementary gates parameterized by the angle $\phi$. Discrete sets of self inverse gates which are universal are also readily constructed. For example, Shi showed that a set comprising the {\sf CNOT} plus any one-qubit gate whose square does not preserve the computational basis is universal \cite{SHI02}. We immediately see that a universal set of self-inverse gates cannot contain only the {\sf CNOT} and a single one-qubit gate. However, the set $\{\text{\sf CNOT}, X,\cos\psi X + \sin\psi Z\}$ is universal for any {\em single} value of $\psi$ which is not a multiple of $\pi/4$.

A reduction from {\sc 5-local} to {\sc 2-local Hamiltonian} was accomplished by the use of \emph{gadgets} that reduced $3$-local Hamiltonian terms to $2$-local terms~\cite{KKR06}.  From the results in~\cite{KKR06} (see also~\cite{OT06}) and the \QMA{}-completeness of \RFLH{}, it now follows that \RH{} is \QMA{}-complete and universal for adiabatic quantum computation. We note that the real product $\PYi\otimes\Yj$, or tensor powers thereof, are not necessary in any part of our construction, and so Hamiltonians composed of the following pairwise products of real-valued Pauli matrices are \QMA{}-complete and universal for adiabatic quantum computation\footnote{The \QMA{}-completeness of this subset of Hamiltonians was found independently by D. Bacon; preprint, (2007).}:
\begin{eqnarray}\label{eqn:resubset}
&&\{{\openone},{\openone}\otimes \X, \openone\otimes\Z,\X\otimes\openone, \\\nonumber
&&~~\Z\otimes\openone,\X\otimes\Z,\Z\otimes\X, \X\otimes\X,\Z\otimes\Z\}.
\end{eqnarray}


To prove our Theorems (1) and (2), we will next show that one can approximate all the terms from~\eqref{eqn:resubset} using either the ZX or ZZXX Hamiltonians---the Hamiltonians from~\eqref{eqn:zzxx} and~\eqref{eqn:zx} respectively.  We do this using perturbation theory~\cite{KKR06,OT06} to construct gadget Hamiltonians that approximate the operators $\Z_i\X_j$ and $\PXi\PZi$ with terms from the ZZXX Hamiltonian as well as the operators $\PZi\PZi$ and $\PXi\Xj$ with terms from the ZX Hamiltonian.


\section{{\scshape XXZZ Hamiltonian} is {\sf QMA}-complete}
